Joint Satellite Gateway Placement and Routing for Integrated Satellite-Terrestrial Networks

With the increasing attention to the integrated satellite-terrestrial networks (ISTNs), the satellite gateway placement problem becomes of paramount importance. The resulting network performance may vary depending on the different design strategies. In this paper, a joint satellite gateway placement and routing strategy for the terrestrial network is proposed to minimize the overall cost of gateway deployment and traffic routing, while adhering to the average delay requirement for traffic demands. Although traffic routing and gateway placement can be solved independently, the dependence between the routing decisions for different demands makes it more realistic to solve an aggregated model instead. We develop a mixed-integer linear program (MILP) formulation for the problem. We relax the integrality constraints to achieve a linear program (LP) which reduces time-complexity at the expense of a sub-optimal solution. We further propose a variant of the proposed model to balance the load between the selected gateways.

==> Satellite Gateway Placement Problem/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we introduce the joint satellite gateway placement and routing problem over an ISTN, for facilitating the terrestrial-satellite communications while adhering to propagation latency requirements, in a cost-optimal manner. %We further, minimize the latency by minimizing the upper bound of the traffic load assigned to each gateway.  
We also balance the corresponding load between selected gateways.To yield a polynomial solution time, we relax the integer variables and derive an LP-based rounding approximation for our model. 

In SDN-enabled ISTNs, the problem of controller placement needs to be addressed mutually with the placement of the satellite-gateways having in mind different design strategies such as cross-layer data delivery, load balancing, reliability and latency optimization, etc. Moreover, instead of placing the satellite gateways on the terrestrial nodes, aerial platforms can be an alternative choice leading to a cross-layer network design problem. The flow routing in this setting is more challenging than the presented work. These two problems are the topics of our future research. 



==> Satellite Gateway Placement Problem/evaluation.tex <==
\section{Performance Evaluation}
\label{sec:evaluation}
In this section we evaluate the performance of our satellite gateway placement method. We first describe the simulation environment setup and scenarios, then we review the performance evaluation results. 
\subsection{Performance Evaluation Setup}
\label{evaluation:setup}
We evaluate the performance of our JSGPR and JSGPR-LB approaches on multiple real network topologies publicly available at the Topology Zoo \cite{zoo}. The five different topologies we consider are listed in table \ref{topo}. The link lengths and capacities are extracted from the topology zoo. The propagation delays are calculated based on the %topology-based nodes distances and 
lengths of the links with the propagation velocity of $C = 2 \times 10 ^8 m/s$ \cite{speed}.  The value of $d_{max}$ is set to $10 ms$, and the deployment cost for each node is taken from a uniform random generator $~U(500, 1000)$. The unit bandwidth cost for all the links is set to be equal to $1$. Also, the value of $q_j$ is set to $240 Mbps$ for all the gateways.
To develop and solve our MILP and LP models we use the CPLEX commercial solver. Our tests are carried out on a server with an Intel i5 CPU at 2.3 GHz and 8 GB of main memory.

% \begin{tabu} to 0.45\textwidth { | X[l] | X[c] | X[r] | }
%  \hline
%  item 11 & item 12 & item 13 \\
%  \hline
%  item 21  & item 22  & item 23  \\
% \hline
%  item 21  & item 22  & item 23  \\
% \hline
%  item 21  & item 22  & item 23  \\
% \hline
%  item 21  & item 22  & item 23  \\
% \hline
% \end{tabu}


\begin{table}[b]
\centering
\begin{tabular}{||c c c||} 
 \hline
 Topology & Nodes & Links  \\ %[0.5ex] 
 \hline\hline
 Sinet & 13 & 18  \\ 
 Ans & 18 & 25  \\
 Agis & 25 & 32  \\
 Digex & 31 & 35  \\
 Bell Canada & 48 & 64 \\ %[1ex] 
 \hline
\end{tabular}
\caption{Summary of the studied topologies}
\label{topo}
\end{table}



\subsection{Evaluation Scenarios}
\label{evaluation:setup}
We have conducted two sets of experiments for two different cases. In the first case we benchmark our LP-based approximation algorithm against the MILP-based optimal one for JSGPR, whereas the second case aims to observe the impact of our load balancing approach on the gateway placement. 
For both cases and for all topologies, if $c^i_{max}$ is the maximum capacity among all the outgoing links of node $i$, the traffic rate originated at node $i$ is taken from a uniform distribution $~ U(\frac{2c^i_{max}}{3}, c^i_{max})$. Specifically, we will use the following metrics to evaluate the performance of our algorithm:

\begin{itemize}
\item \textbf{Solver Runtime} is the amount of time the CPLEX solver takes to solve the generated MILP or LP instances.  
\item \textbf{Average Delay} as explained in section \ref{sec:desc}.
\item \textbf{Total Cost} is the total cost of deploying the satellite gateways and routing the traffic.
\item \textbf{Gateway Load} is the amount of traffic assigned to the gateways after the gateway placement problem is solved.
% \item \textbf{Link Utilization} is the overall amount of traffic passed through a network link to satisfy the network traffic demand.
\end{itemize}

\subsection{Evaluation Results}
\label{sec3}
\begin{figure*}[t]
\begin{center}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/costGW.png}
\caption{Exp-A: Normalized Total Cost}
\label{fig:acc}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/time.png}
\caption{Exp-A: Average Solver Runtime}
\label{fig:util}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/digex_time_bp.png}
\caption{Exp-A: Solver Runtime for Digex}
\label{fig:prev}
\end{minipage}
\hspace{1em}

% %The following will be removed.
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{figures/digex_delay_bp.png}
% \caption{Exp-A: Average Latency for Digex}
% \label{fig:bwrev}
% \end{minipage}
% \hspace{1em}
% %The following will be removed.
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{figures/Ans_delay_bp.png}
% \caption{Exp-A: Average Latency for Ans}
% \label{fig:bwrev2}
% \end{minipage}
% \hspace{1em}

%The two above will be replaced by the following:
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{results/ICC2020/Ans_delay_bp.png}
% \caption{Exp-A: Average Latency for Ans}
% \label{fig:bwrev2}
% \end{minipage}
% \hspace{1em}
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{results/ICC2020/Agis_delay_bp.png}
% \caption{Exp-A: Average Latency for Agis}
% \label{fig:bwrev2}
% \end{minipage}
% \hspace{1em}
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{results/ICC2020/Digex_delay_bp.png}
% \caption{Exp-A: Average Latency for Digex}
% \label{fig:bwrev2}
% \end{minipage}
% \hspace{1em}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/Agg_delay_bp.png}
\caption{Exp-A: Average Delay ($d_{max} = 10 ms$ )}
\label{fig:agg}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/perdelay.png}
\caption{Exp-A: Total Cost with Varying Delay Bound}
\label{fig:comp}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/costload.png}
\caption{Exp-B: Normalized Total Cost}
\label{fig:cost2}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.225\textwidth}
\includegraphics[width=1\linewidth]{results/ICC2020/Agg_load_bp.png}
\caption{Exp-B: Gateway Load }
\label{fig:load_profile}
\end{minipage}
\hspace{1em}
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{results/ICC2020/sinet_load_bp.png}
% \caption{Exp-B: Comparison of Maximum Gateway Load for Sinet}
% \label{fig:load1}
% \end{minipage}
% \hspace{1em}
% \begin{minipage}[h]{0.225\textwidth}
% \includegraphics[width=1\linewidth]{results/ICC2020/ans_load_bp.png}
% \caption{Exp-B: Comparison of Maximum Gateway Load for Ans}
% \label{fig:load2}
% \end{minipage}

\end{center}
\end{figure*}

\subsubsection{Experiment A - Approximation vs. Exact Method}Fig. \ref{fig:acc} reflects the average normalized total cost for both the optimal MILP-based approach and the LP-based approximation of JSGPR. Due to the suboptimal placement, the LP-based approach results in additional deployment costs within the range of at most $13\%$ of the optimal placement, but as the scale of the network gets larger this gap decreases. For Digex the approximate approach leads to about $4\%$ increase in the deployment cost. 

Fig. \ref{fig:util} depicts the average runtime for both the MILP and LP formulations for the $4$ topologies. We note that for larger networks, CPLEX failed to provide the solution for the MILP problem, while our LP model continued to solve the problem within the expected time limit. Particularly, for the Bell-Canada topology, in $40\%$ of the runs, CPLEX was not able to find any feasible solutions within the first $10$ hours while the approach via approximation could provide the suboptimal placement in less than $15$ minutes. The solver runtime for Digex is shown in \ref{fig:prev}. The average runtime for the LP is $230$ seconds while for the MILP, it is around $3000$ seconds.

% Fig. \ref{fig:bwrev}, and \ref{fig:bwrev2} show the average latency profile for the the exact approach and the approximation for Digex and Ans. The link density, and the capacity of the links in each topology have impacts on the delay profiles, but in each case the average delay was within the specified range. 
Fig. \ref{fig:agg}, represents the average delay for Ans, Agis, and Digex. The average of the expected experienced delay under the MILP model is $2.95, 6.18,$ and $ 2.15$ seconds, while this value under the LP model is $4.68, 5.6,$ and $1.65$ seconds. We note that the suboptimal procedure leads to additional deployed gateways in Agis and Digex, which in return will have the nodes end up closer to the gateways and consequently, experience lower average delay.
Further, an insightful observation is that, in Agis, $d_{max}$ is relatively a tight upper bound on the average delay experienced by each node. Therefore, the delay profile is pushed towards its upper bound, whereas, in Digex, due to the low density of links, more gateways are required to be deployed on the terrestrial nodes, which will make the gateways available more quickly; Therefore, the delay profile is inclined towards its lower bound.    

Fig. \ref{fig:comp} depicts the normalized cost of the JSGPR problem for different values of $d_{max}$. For instance, as indicated by this figure, if in Digex, a delay of $10 ms$ is tolerable instead of $2ms$, a $35\%$ reduction in cost results; Similarly, upgrading the service from a delay of $5ms$ to $2ms$ in Agis, will almost double the cost.

Overall, the aforementioned figures illustrate that the performance of our approximation algorithm is very close to the exact approach, but with an important advantage of reduced time complexity which shows the efficiency of our proposed approximation method.

\subsubsection{Experiment B - The Impact of Load Minimization}
Fig. \ref{fig:cost2} shows the profile of the average load on the gateways for JSGPR, %JSGPR-NC, 
and JSGPR-LB, considering the Agis and Digex topologies. As expected, JSGPR-LB is more costly, since in order to evenly share the load between the gateways, %and minimize the maximum of the load on the gateways, 
a larger number of gateways will be required. %It is interesting that the cost of JSGPR and JSGPR-NC is almost equal. The reason is that the maximum capacity of $240 Mbps$ for a terrestrial-satellite link is high enough to be alleviated relative to the load assigned to the gateways. therefore the corresponding constraint will be redundant. 

Fig. \ref{fig:load_profile} depicts the profile of the load assigned to the gateways. In both depicted topologies, the load profile under JSGPR-LB is very thin and concentrated over its average, proving the efficiency of the formulation. %Moreover, the load profile Unde JSGPR and JSGPR-NC is almost the same for Digex which aligns with our intuition and with the consequences of Fig. \ref{fig:cost2}. 
Lower load on the placed gateways is achieved by the sub-optimal placement of the gateways (due to the larger number of gateways) which results in a more expensive gateway placement. As depicted in Fig. \ref{fig:cost2} the total cost of gateway placement in the studied topologies %by JSGPR-LB is an upper bound to that of JSGPR. More precisely, the resulted cost under 
for JSGPR-LB is above and within the range of $16\%$ of the optimal placement cost achieved by JSGPR.

==> Satellite Gateway Placement Problem/formulation_old.tex <==
\section{Problem Formulation}
\label{sec:problem}
\subsection{JSGPR MILP Formulation}
In order to formulate the JSGPR problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the traffic rate passing through the link $(u,v)$ corresponding to flow $i\rightarrow j$.
\end{itemize}

The MILP formulation is as follows:
%as a mixed integer-linear program (MILP) which will follow. 

% \vspace{2mm}
% \noindent\textbf{Objective function:}
% \begin{equation}
%     \textbf{Minimize} \quad \sum_{i\in V}{x_i} + 1/N\sum_{n \in V}\sum_{ij \in E}{z_n^{ij}d_{ij}}
% \end{equation}

% \begin{equation}
%     \sum_{i \in V}{y_{ij}} = 1,\; \quad \forall j \in V
% \end{equation}

% \begin{equation}
%     y_{ij}\leq x_i, \; \quad \forall i,j \in V
% \end{equation}

% \begin{equation}
%     \sum_{iv \in E}{z^{iv}_{j}} - \sum_{ui \in E}{z^{ui}_{j}}  = y_{ij}. \; \quad \forall i,j \in V
% \end{equation}

% \vspace{2mm}
% \noindent\textbf{Objective: }
% \begin{equation}
%     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
% \end{equation}


% \noindent\textbf{Demand Guarantee Constraints: }
% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
% \end{equation}

% \noindent\textbf{Feasibility Guarantee Constraints: }
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}a_ix_{ij} \leq b_jy_j,\; \quad \forall j \in J 
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq a_ix_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Link Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
% \end{equation}

% \noindent\textbf{Flow Constraints: }
% \begin{equation}
%     \quad a_ix_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + a_ix_{iu}, \; \\ 
%         & \quad \forall i \in I, u \in V,  u \neq i
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

% \begin{equation}
%     \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
% \end{equation}

% \begin{equation}
%     \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
% \end{equation}


% \newpage

\vspace{2mm}
\noindent\textbf{Objective: }
\begin{equation}
    \textbf{Minimize} \quad%(1-\phi)%
    \sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv} \;
    \label{obj}
    %     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j}\;
    % \label{obj}
\end{equation}


\noindent\textbf{Demand Guarantee Constraints: }
\begin{equation}
    \quad\sum_{j \in J}\sum_{u \in V} f^{ij}_{uj} = a_i,\; \quad \forall i \in I 
    \label{demgar}
\end{equation}

\noindent\textbf{Feasibility Guarantee Constraints: }
\begin{equation}
    \quad \sum_{u \in V} f^{ij}_{uj} \leq y_j a_i,\; \quad \forall i \in I, \forall j \in J 
    \label{leq}
\end{equation}

\noindent\textbf{Delay Guarantee Constraints:}
\begin{equation}
    \quad \sum_{j \in J}\sum_{uv \in L}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
    \label{delgar}
\end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq b_jy_j,\; \quad \forall j \in J 
%     \label{cap}
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq \sum_{u \in V} f^{ij}_{uj},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
%     \label{maxflow}
% \end{equation}

\noindent\textbf{Link Capacity Constraints: }
\begin{equation}
    \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
    \label{linkcap}
\end{equation}

\noindent\textbf{Flow Constraints: }
\begin{equation}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad f^{ii}_{ii} + \sum_{v\in V: iv \in L}\sum_{j\neq i \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1}
\end{equation}

\begin{equation}
    \begin{aligned}
        % &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + \sum_{u \in V} f^{iu}_{uu}, \; \\ 
        % & \quad \forall i \in I, u \in V,  u \neq i
        &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} \; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i
    \end{aligned}
    \label{flow2}
\end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1}
\end{equation}

\begin{equation}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
    \label{dom2}
\end{equation}

\vspace{2mm}
% The first term of the objective function \eqref{obj} is the cost associated with the deployment of the gateways while the second term is the average end-to-end delay of all the flows which traverse the network.  We aim at minimizing the objective function seeking a trade-off between the two terms. The trade-off factor in the objective function is denoted by $\phi$.
The objective function \eqref{obj} is the total cost of the process, consisting of the gateway deployment cost and the bandwidth cost
Constraints \eqref{demgar} are to ensure that the traffic demand for each node is satisfied using one or multiple gateways. Constraints \eqref{leq} allow for the formation of the flow $i\rightarrow j$ only if a gateway is placed at node $j$, while constraints \eqref{delgar} will guarantee that the average end-to-end delay for each demand point will not exceed a pre-defined upper bound $d_{max}$.
% , while constraints \eqref{cap} ensure that the load on each gateway is less than the capacity of the gateway (i.e. less than the capacity of the gateway-satellite node.)
% By constraints \eqref{maxflow}, the rate that each link $(u,v)$ allocates to flow $i\rightarrow j$ is at most equal to the part of the demand of node $i$ which gateway $j$ is responsible for. 
Constraints \eqref{linkcap} make sure that the resources allocated by each link does not exceed the capacity of that link. Constraints \eqref{flow1} and \eqref{flow2}  enforce the flow conservation; i.e. the inbound traffic to a switch must be equal to its outbound traffic. Finally, the  constraints \eqref{dom1}, and \eqref{dom2} express the domain requirements for the variables $\textbf{y}$, and $\textbf{f}$ respectively.

% We also define another notation which does not show up in the problem setup but becomes useful for further discussions. Let $\textbf{x}$ be a set of $x_{ij}$ variables which represent the portion of the traffic originated by node $i$ which is going to be gatewayed to the satellite through gateway $j$. More precisely we write: 
% \begin{equation}
%     x_{ij} = \frac{\sum_{u \in V}{f^{ij}_{uj}}}{a_i}
%     \label{aux}
% \end{equation}
% Where $0\leq x_{ij}\leq1$. Utilizing \eqref{aux}, a few of the constraints in the above-mentioned minimization problem, including \eqref{demgar}, and \eqref{leq}, could be written in the somewhat more intuitive following form:

% % and \eqref{maxflow}, 

% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
%     \label{aux1}
% \end{equation}
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J
%     \label{aux2}
% \end{equation}
% % \begin{equation}
% %     \quad f^{ij}_{uv} \leq a_i x_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% %     \label{aux3}
% % \end{equation}

% With this alternative notation, the formulated problem very much looks like a variant of the facility location problem formulated in \cite{Bell}; Utilizing the flow variables in the described fashion allows for path splitting which improves the flexibility of the network, and the efficiency of link usage.

Since the MILP is known to be NP-hard, the proposed formulation is intractable for larger scale networks. Next we derive an LP model to strike a balance between the time-complexity of the optimization problem and the accuracy of the results.   


% %TABLE///////////////////%

% \begin{table}[h]
% \centering
% \label{table}
% \begin{center}
% {
% \begin{tabularx}{\textwidth}{|c|X|}

% \hline
% Variables & Description\\
% \hline
% %$q_l[i]$ & Location of the UAV l at timeslot i\\
% $y_j$ & Binary variable determining whether or not a gateway is placed at node $j$. \\
% % $ $ & kjh\\
% $x_{ij}$ & Continuous variable in [0, 1] determining the portion of demanded traffic for node i, which is routed through node j. \\
% $f_{uv}^{ij}$ & The flow passing through the link $(u,v)$ corresponding to node $i$ destined at gateway j.\\
% \hline
% Parameters & Description\\
% \hline
% $a_i$ & Overall traffic generated at node $i$ \\
% $c_j$ & The cost of placing a gateway at node $j$\\
% $d_{uv}$ & The delay corresponding to routing packets through the link $(u,v)$\\
% $q_{uv}$, &Flow capacity of the link $(u,v)$ \\
% %$\rho_0$ & Channel power gain at the reference distance of 1m\\
% %$\gamma_{min}$ & Minimum received SNR for a successful transmission\\
% %$\sigma_n^2$ & Thermal noise power\\
% %$E$ & Transmission power of the nodes\\
% %$d_{min}$ & minimum allowed distance between two UAVs\\
% \hline
% \end{tabularx}}
% \end{center}
% \caption{Variables and Parameters Description}
% \end{table}
\subsection{LP Relaxation and Rounding Algorithm}

The LP model is obtained from the original MILP formulation by relaxing the integrality of the binary $\textbf{y}$ variables. We replace the domain constraints \eqref{dom1} by the following ones:

\begin{equation}
    \quad y_{j} \in [0, 1],\; \quad \forall j \in J
    \label{domain1new}
\end{equation}

The rest of the model remains intact. The LP model can be solved within a polynomial effort, but does not necessarily leave us with a valid gateway placement. Therefore, inspired by \cite{torkzaban2019trust}, we use a deterministic rounding algorithm to derive binary values for the $\textbf{y}$  placement variables, with the cost of solution suboptimality. The rounding is pseudo-coded in \textbf{Algorithm-\ref{alg}}, and works as follows; In each iteration (Lines \ref{2}-\ref{11}), first an LP model is solved, then the value $y_j$ for each satellite gateway candidate is extracted as presented in the line \ref{6}. Then the candidate corresponding to the maximum  $y_j$ is chosen to be rounded to $1$ and added to the LP model (Lines \ref{6}-\ref{8}). Since the $y_j$ variables only show up in the right half-side of the $(\leq)$constraints, non of the constraints get violated by this choice. The algorithm terminates after all the dimensions of the solution are rounded (i.e. no fractional values show up in the solution of the LP model), or when the LP model becomes infeasible in which case the gateway placement is denied. After the placement of the gateways is determined, a multi-commodity flow (MCF) allocation algorithm is run to find out the corresponding flow variables. 

Since the integral part of the solution has at most $|J|$ dimensions, the $\textbf{Solve\_LP(..)}$ function will run at most $|J|$ times which results in a polynomial time-complexity as stated earlier.
% We also note that in the calculation of $\lambda_j$, the product of $y_j$ and the total load on $jth$ gateway candidate, i.e. $\sum_{i\in I}{a_ix_{ij}}$ is obtained instead of merely considering the relaxed $y_j$ placement variables. This way a gateway candidate that both has a high fractional placement value, and a high amount of assigned load, is preferred to be chosen in the final placement choice.  


\begin{algorithm}
\caption{LP Rounding}
\label{alg}
\begin{algorithmic}[1]


\REPEAT \label{1}
    \STATE $\{y_j, f^{ij}_{uv}\} \leftarrow \textbf{Solve\_LP(..)}$ \label{2}

    \STATE If solution exists \textit{Sol:= true}, Otherwise \textit{Sol:= false} \label{3}

    \STATE  $Y \leftarrow\{y_j |y_j \notin \{0, 1\} \}$ \label{4}
    
   \IF{$Y \neq 0$} \label{5} 
   % \STATE  $X_a \leftarrow\{x^i_u |x^i_u \in X  \land g_{i} <= r_{u} \}$

    %\IF{$X_a \neq 0$}
  %   \STATE $\{i_0, u_0\} \leftarrow argmax_{\{i \in V_f, u \in V_s\}} X_a $
    % \STATE $\Lambda := \{\lambda_j:=y_j*(\sum_{i\in I}{x_{ij}})|j \in J\}$ \label{new}
    \STATE $\{y_0\} \leftarrow \arg \max_{\{j \in J\}} Y $ \label{6}
    % \IF{$\{i_0, u_0\}$ exists} \label{7}
    \STATE \textbf{Add LP Constraint $y_0=1$} \label{8}
    % \ELSE \label{9}
    % \STATE \textit{Sol=false} \label{10}
    \ENDIF \label{11}
    % \ENDIF \label{12}
\UNTIL $(Y=0) \lor(Sol =false)$ \label{13}   
%\UNTIL $(X=0) \lor (X_a=0) \lor   (Sol =false)$

\IF{$Sol= true$} \label{14}
\STATE $\{y_j, f^{ij}_{uv}\} \leftarrow \textbf{Solve\_MCF(..)}$ \label{15}

    \STATE If solution exists \textit{Sol:= true}, Otherwise \textit{Sol:= false} \label{16}
\ENDIF \label{26}
%    \IF{\textit{Sol:= true}} \label{17}
%\RETURN $\{x^i_u, f^{ij}_{uv}\}$ \{Accept the request\} \label{18}
%    \ELSE \label{19}
%    \STATE $\{\forall{x^i_u} :=0, \forall{f^{ij}_{uv}} :=0\}$ \label{20}
%   \RETURN $\{x^i_u, f^{ij}_{uv}\}$ \{Deny the request\} \label{21}
%    \ENDIF \label{22}
%\ELSE \label{23}
%\STATE $\{\forall{x^i_u} :=0, \forall{f^{ij}_{uv}} :=0\}$ \label{24}
%\RETURN $\{x^i_u, f^{ij}_{uv}\}$ \{Deny the request\} \label{25}
\IF{\textit{Sol:= true}} \label{17}
\RETURN $\{y_j, f^{ij}_{uv}\}$ \{Accept the placement\} \label{18}
\ELSE \label{19}
\STATE $\{\forall{y_j} :=0, \forall{f^{ij}_{uv}} :=0\}$ \label{20}
\RETURN $\{y_j, f^{ij}_{uv}\}$ \{Reject the placement\} \label{21}
\ENDIF \label{22}


\end{algorithmic}
\end{algorithm}

% Since after solving the LP model, the fractional resulting variables do not determine a valid placement for the gateways, we use a deterministic LP-based rounding algorithm to derive integer values for variables.

% \subsection{Load Balancing}
% To balance the flow on the gateways we inject a new constraint to the model. We will force the load difference between any two potential gateways to be less than a certain amount. We refer to this amount by $load_thr$ which is set prior to design of the model. The constraint that carries our load balancing requirement is represented in the following set of constraint: 

% \begin{equation}
%   y_jy_k |\sum_{i\in I}{a_ix_{ij}}-\sum_{i\in I}{a_ix_{ik}}| \leq thr\; \quad \forall j,k\in J
% \end{equation}
% To linearize the above constraint, we introduce a large enough constant $M$ and rewrite the above set of constraints as the two following ones.


% \begin{equation}
%     \sum_{i\in I}{a_ix_{ij}}-\sum_{i\in I}{a_ix_{ik}} \leq (2- y_j-y_k)M + thr\; \quad \forall j,k\in J
% \end{equation}

% \begin{equation}
%         \sum_{i\in I}{a_ix_{ik}}-\sum_{i\in I}{a_ix_{ij}} \leq (2- y_j-y_k)M + thr\; \quad \forall j,k\in J
% \end{equation}
% The constraints imply that for any two pair of gateways the load difference is less than the maximum value allowed, otherwise the constraints are void. 

\subsection{JSGPR-LM MILP Formulation}

We define a new term $l_{max}$ to represent the maximum of assigned traffic to a gateway, among all the gateways in the optimal placement. In order to minimize the forwarding latency we wish to minimize the value of $l_{max}$. Hence, we will add $l_{max}$ as an additional term to the objective function. The new objective function will look like: 

\begin{equation}
    % \textbf{Minimize} \quad(1-\phi)\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
    % \label{obj}
        \textbf{Minimize} \quad(\sum_{j \in J}c_jy_{j}+\phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}) + \alpha l_{max}\;
    \label{objlm}
\end{equation}

Where $\alpha$ is a constant factor determining the balance between the two terms of the objective function. To ensure that the traffic assigned to each gateway does not exceed $l_{max}$, we add the following set of constraints to our model:

\begin{equation}
         \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq l_{max}\; \quad \forall j \in J 
\end{equation}

The resulted optimization problem aims to minimize the load of the gateways in conjunction with the cost of the gateway deployment. 

==> Satellite Gateway Placement Problem/formulation_old2.tex <==
\section{Problem Formulation}
\label{sec:problem}
\subsection{Satellite GW placement problem MILP Formulation I as CFLP}
In order to formulate the  problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{x}$, where $x_{ij}$ expresses the fraction of traffic demand originating at $i$ passing through gateway $j$.
\end{itemize}

 \vspace{2mm}
 \noindent\textbf{Objective function:}
 \begin{equation}
     \textbf{Minimize} \quad \sum_{j\in J}c_j {y_j} + \sum_{i \in I}\sum_{j \in J}{c_{ij} a_{i}x_{ij}}
 \end{equation}

 \begin{equation}
     \sum_{i \in V}{x_{ij}} = 1,\; \quad \forall j \in V
     \label{c1}
 \end{equation}

 \begin{equation}
     x_{ij}\leq y_j, \; \quad \forall i,j \in V
     \label{c2}
 \end{equation}
 
  \begin{equation}
     \sum_{i \in V}a_i {x_{ij}} \leq q_j y_j,\; \quad \forall j \in V
     \label{c3}
 \end{equation}

\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1a}
\end{equation}

\begin{equation}
    \quad 1 \geq x_{ij} \geq 0,\; \quad \forall i \in I, j \in J
    \label{dom2a}
\end{equation}


The objective function minimizes the total cost; which comprises of two terms: the first one represents the cost of installing and opening a gw where $c_j$ denotes the cost of installing and opening a gw at location $j$, the second term accounts for the demand allocation cost, 
where $c_{ij}$ denotes the cost of supplying by gw j the fraction $x_{ij}$  of the demand $a_i$ originating at $i$. Constraint set \ref{c1} assures that traffic demands are supported through the gws, while constraint set \ref{s2} assures that demands are only served by open gws. Constraints \ref{c3} state the capacity constraints for the facilities. The domains of yi and xij variables are defined in constraints \ref{dom1} and \ref{dom2}, respectively. The UFLP is modeled by dropping constraints \ref{c3}.

\subsection{Satellite GW placement problem and routing MILP Formulation I as CFLP}
In order to formulate the  problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{x}$, where $x_{ij}$ expresses the fraction of traffic demand originating at $i$ passing through gateway $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the amount of traffic demand originating at $i$ assigned to gateway $j$ passing through the link $(u,v)$.
\end{itemize}
 \vspace{2mm}
 \noindent\textbf{Objective function:}
 \begin{align}
     \textbf{Minimize} \quad \sum_{j\in J}c_j {y_j} + \sum_{i \in I}\sum_{j \in J}{c_{ij} a_{i}x_{ij}} + \sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}
 \end{align}
 \noindent\textbf{Demand Constraints:}
 \begin{align}
     \sum_{i \in V}{x_{ij}} = 1,\; \quad \forall j \in V
     \label{c1b}
 \end{align}
 \noindent\textbf{Feasibility Constraints:}
 \begin{align}
     x_{ij}\leq y_j, \; \quad \forall i,j \in V
     \label{c2b}
 \end{align}
\begin{align}
     f_{uv}^{ij} \leq a_i x_{ij}, \; \quad \forall i,j \in V
     \label{c3b}
 \end{align}
  \noindent\textbf{Capacity Constraints:}
  \begin{align}
     \sum_{i \in V}a_i {x_{ij}} \leq q_j y_j,\; \quad \forall j \in V
     \label{c4b}
 \end{align}
 \begin{align}
     \sum_{i \in V} \sum_{j \in V} f_{uv}^{ij}  \leq q_{uv}\; \quad \forall j \in V
     \label{c5b}
 \end{align}
  \noindent\textbf{Flow Constraints: }
 \begin{align}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad a_i x_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1b}
\end{align}
\begin{align}
        &\quad \sum_{v \in V: (v,u) \in L}\sum_{j\in J}f^{ij}_{vu} - \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} = a_i x_{iu}\; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i
    \label{flow2b}
\end{align}
%%%%%%%%%%%%%%%%%%
\noindent\textbf{Domain Constraints: }
\begin{align}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1b}
\end{align}
\begin{align}
    \quad  x_{ij} \in \{0, 1\},\; \quad \forall i \in I, j \in J
    \label{dom2b}
\end{align}
\begin{align}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
    \label{dom3b}
\end{align}

The objective function minimizes the total cost; which comprises of three terms; the first one represents the cost of installing and opening a gw at location $j$. The second term accounts for the demand allocation cost, where $c_{ij}$ denotes the cost of supplying by gw j the fraction $x_{ij}$  of the demand $a_i$ originating at $i$. The last term corresponds to the transport/connection cost from the demand originating at $i$ to its assigned gw $j$, 

Constraints set \ref{c1b} assures that traffic demands are supported by the selected gateways. Feasibility constraints set \ref{c2b} make sure that demands are only served by open gateways, while in \ref{c3b} the amount of traffic from the demand originating at $i$ assigned to gateway $j$ passing through the link $(u,v)$ cannot exceed the requested traffic demand $a_i$.  Constraints \ref{c4b} and \ref{c5b} state the capacity constraints for the gateways and the links. Constraints \ref{flow1b} and ref{flow2b} enforce the flow conservation.
The domains of $y_i$, $x_{ij}$ and $f_{uv}^{ij}$ variables are defined in constraints \ref{dom1}, \ref{dom2}, \ref{dom3}, respectively. 

In the aforementioned formulation we can alleviate the constraints set \ref{c4b} if we do not consider any other (e.g., maximum CPU load) on the potential gateways, as well as the $2^{nd}$ term of the objective function if there is no demand allocation cost.





//////////////////////////////////////////////////////
\subsection{JSGPR MILP Formulation II}
In order to formulate the JSGPR problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the traffic rate passing through the link $(u,v)$ corresponding to flow $i\rightarrow j$.
\end{itemize}

The MILP formulation is as follows:
%as a mixed integer-linear program (MILP) which will follow. 

% \vspace{2mm}
% \noindent\textbf{Objective function:}
% \begin{equation}
%     \textbf{Minimize} \quad \sum_{i\in V}{x_i} + 1/N\sum_{n \in V}\sum_{ij \in E}{z_n^{ij}d_{ij}}
% \end{equation}

% \begin{equation}
%     \sum_{i \in V}{y_{ij}} = 1,\; \quad \forall j \in V
% \end{equation}

% \begin{equation}
%     y_{ij}\leq x_i, \; \quad \forall i,j \in V
% \end{equation}

% \begin{equation}
%     \sum_{iv \in E}{z^{iv}_{j}} - \sum_{ui \in E}{z^{ui}_{j}}  = y_{ij}. \; \quad \forall i,j \in V
% \end{equation}

% \vspace{2mm}
% \noindent\textbf{Objective: }
% \begin{equation}
%     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
% \end{equation}


% \noindent\textbf{Demand Guarantee Constraints: }
% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
% \end{equation}

% \noindent\textbf{Feasibility Guarantee Constraints: }
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}a_ix_{ij} \leq b_jy_j,\; \quad \forall j \in J 
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq a_ix_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Link Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
% \end{equation}

% \noindent\textbf{Flow Constraints: }
% \begin{equation}
%     \quad a_ix_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + a_ix_{iu}, \; \\ 
%         & \quad \forall i \in I, u \in V,  u \neq i
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

% \begin{equation}
%     \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
% \end{equation}

% \begin{equation}
%     \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
% \end{equation}


% \newpage

\vspace{2mm}
\noindent\textbf{Objective: }
\begin{equation}
    \textbf{Minimize} \quad%(1-\phi)%
    \sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv} \;
    \label{obj}
    %     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j}\;
    % \label{obj}
\end{equation}


\noindent\textbf{Demand Guarantee Constraints: }
\begin{equation}
    \quad\sum_{j \in J}\sum_{u \in V} f^{ij}_{uj} = a_i,\; \quad \forall i \in I 
    \label{demgar}
\end{equation}

\noindent\textbf{Feasibility Guarantee Constraints: }
\begin{equation}
    \quad \sum_{u \in V} f^{ij}_{uj} \leq y_j a_i,\; \quad \forall i \in I, \forall j \in J 
    \label{leq}
\end{equation}

\noindent\textbf{Delay Guarantee Constraints:}
\begin{equation}
    \quad \sum_{j \in J}\sum_{uv \in L}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
    \label{delgar}
\end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq b_jy_j,\; \quad \forall j \in J 
%     \label{cap}
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq \sum_{u \in V} f^{ij}_{uj},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
%     \label{maxflow}
% \end{equation}

\noindent\textbf{Link Capacity Constraints: }
\begin{equation}
    \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
    \label{linkcap}
\end{equation}

\noindent\textbf{Flow Constraints: }
\begin{equation}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad f^{ii}_{ii} + \sum_{v\in V: iv \in L}\sum_{j\neq i \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1}
\end{equation}

\begin{equation}
    \begin{aligned}
        % &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + \sum_{u \in V} f^{iu}_{uu}, \; \\ 
        % & \quad \forall i \in I, u \in V,  u \neq i
        &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} \; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i
    \end{aligned}
    \label{flow2}
\end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1}
\end{equation}

\begin{equation}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
    \label{dom2}
\end{equation}

\vspace{2mm}
% The first term of the objective function \eqref{obj} is the cost associated with the deployment of the gateways while the second term is the average end-to-end delay of all the flows which traverse the network.  We aim at minimizing the objective function seeking a trade-off between the two terms. The trade-off factor in the objective function is denoted by $\phi$.
The objective function \eqref{obj} is the total cost of the process, consisting of the gateway deployment cost and the bandwidth cost
Constraints \eqref{demgar} are to ensure that the traffic demand for each node is satisfied using one or multiple gateways. Constraints \eqref{leq} allow for the formation of the flow $i\rightarrow j$ only if a gateway is placed at node $j$, while constraints \eqref{delgar} will guarantee that the average end-to-end delay for each demand point will not exceed a pre-defined upper bound $d_{max}$.
% , while constraints \eqref{cap} ensure that the load on each gateway is less than the capacity of the gateway (i.e. less than the capacity of the gateway-satellite node.)
% By constraints \eqref{maxflow}, the rate that each link $(u,v)$ allocates to flow $i\rightarrow j$ is at most equal to the part of the demand of node $i$ which gateway $j$ is responsible for. 
Constraints \eqref{linkcap} make sure that the resources allocated by each link does not exceed the capacity of that link. Constraints \eqref{flow1} and \eqref{flow2}  enforce the flow conservation; i.e. the inbound traffic to a switch must be equal to its outbound traffic. Finally, the  constraints \eqref{dom1}, and \eqref{dom2} express the domain requirements for the variables $\textbf{y}$, and $\textbf{f}$ respectively.

% We also define another notation which does not show up in the problem setup but becomes useful for further discussions. Let $\textbf{x}$ be a set of $x_{ij}$ variables which represent the portion of the traffic originated by node $i$ which is going to be gatewayed to the satellite through gateway $j$. More precisely we write: 
% \begin{equation}
%     x_{ij} = \frac{\sum_{u \in V}{f^{ij}_{uj}}}{a_i}
%     \label{aux}
% \end{equation}
% Where $0\leq x_{ij}\leq1$. Utilizing \eqref{aux}, a few of the constraints in the above-mentioned minimization problem, including \eqref{demgar}, and \eqref{leq}, could be written in the somewhat more intuitive following form:

% % and \eqref{maxflow}, 

% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
%     \label{aux1}
% \end{equation}
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J
%     \label{aux2}
% \end{equation}
% % \begin{equation}
% %     \quad f^{ij}_{uv} \leq a_i x_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% %     \label{aux3}
% % \end{equation}

% With this alternative notation, the formulated problem very much looks like a variant of the facility location problem formulated in \cite{Bell}; Utilizing the flow variables in the described fashion allows for path splitting which improves the flexibility of the network, and the efficiency of link usage.

Since the MILP is known to be NP-hard, the proposed formulation is intractable for larger scale networks. Next we derive an LP model to strike a balance between the time-complexity of the optimization problem and the accuracy of the results.   


% %TABLE///////////////////%

% \begin{table}[h]
% \centering
% \label{table}
% \begin{center}
% {
% \begin{tabularx}{\textwidth}{|c|X|}

% \hline
% Variables & Description\\
% \hline
% %$q_l[i]$ & Location of the UAV l at timeslot i\\
% $y_j$ & Binary variable determining whether or not a gateway is placed at node $j$. \\
% % $ $ & kjh\\
% $x_{ij}$ & Continuous variable in [0, 1] determining the portion of demanded traffic for node i, which is routed through node j. \\
% $f_{uv}^{ij}$ & The flow passing through the link $(u,v)$ corresponding to node $i$ destined at gateway j.\\
% \hline
% Parameters & Description\\
% \hline
% $a_i$ & Overall traffic generated at node $i$ \\
% $c_j$ & The cost of placing a gateway at node $j$\\
% $d_{uv}$ & The delay corresponding to routing packets through the link $(u,v)$\\
% $q_{uv}$, &Flow capacity of the link $(u,v)$ \\
% %$\rho_0$ & Channel power gain at the reference distance of 1m\\
% %$\gamma_{min}$ & Minimum received SNR for a successful transmission\\
% %$\sigma_n^2$ & Thermal noise power\\
% %$E$ & Transmission power of the nodes\\
% %$d_{min}$ & minimum allowed distance between two UAVs\\
% \hline
% \end{tabularx}}
% \end{center}
% \caption{Variables and Parameters Description}
% \end{table}


\subsection{JSGPR-LM MILP Formulation}

We define a new term $l_{max}$ to represent the maximum of assigned traffic to a gateway, among all the gateways in the optimal placement. In order to minimize the forwarding latency we wish to minimize the value of $l_{max}$. Hence, we will add $l_{max}$ as an additional term to the objective function. The new objective function will look like: 

\begin{equation}
    % \textbf{Minimize} \quad(1-\phi)\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
    % \label{obj}
        \textbf{Minimize} \quad(\sum_{j \in J}c_jy_{j}+\phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}) + \alpha l_{max}\;
    \label{objlm}
\end{equation}

Where $\alpha$ is a constant factor determining the balance between the two terms of the objective function. To ensure that the traffic assigned to each gateway does not exceed $l_{max}$, we add the following set of constraints to our model:

\begin{equation}
         \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq l_{max}\; \quad \forall j \in J 
\end{equation}

The resulted optimization problem aims to minimize the load of the gateways in conjunction with the cost of the gateway deployment. 

==> Satellite Gateway Placement Problem/formulations.tex <==
\section{Problem Formulation}
\label{sec:problem}

\subsection{JSGPR MILP Formulation I}
Inspired by \cite{Bell}, we formulate a baseline for the JSGPR problem as the capacitated facility location-routing problem considering: 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{x}$, where $x_{ij}$ expresses the fraction of traffic demand originating at $i$ passing through gateway $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the amount of traffic demand originating at $i$, assigned to gateway $j$ passing through the link $(u,v)$.
\end{itemize}
 \vspace{2mm}
 We note that for a gateway $u$, the variable $f_{uu}^{iu}$ represents the amount of traffic which is originated at node $i$ and is forwarded to the satellite through the gateway placed at node $u$. 
%  \noindent\textbf{Objective function:}

The resulting MILP formulation is as follows:
 \begin{align}
     \textbf{Minimize} \quad \sum_{j\in J}c_j {y_j} + %\sum_{i \in I}\sum_{j \in J}{c_{ij} a_{i}x_{ij}} + 
     \sum_{i \in I}\sum_{j \in J}\sum_{(u,v) \in E}c_{uv}f^{ij}_{uv}
 \end{align}
 \noindent\textbf{Demand Constraints:}
 \begin{align}
     \sum_{j \in J}{x_{ij}} = 1,\; \quad \forall i \in I
     \label{c1b}
 \end{align}
 \noindent\textbf{Feasibility Constraints:}
 \begin{align}
     x_{ij}\leq y_j, \; \quad \forall i\in I, j \in J
     \label{c2b}
 \end{align}
%  \begin{align}
%       f_{uv}^{ij} \leq a_i x_{ij}, \; \quad \forall i\in I, j \in J
%       \label{c3b}
%   \end{align}
  \noindent\textbf{Capacity Constraints:}
  \begin{align}
     \sum_{i \in I}a_i {x_{ij}} \leq q_j y_j,\; \quad \forall j \in J
     \label{c4b}
 \end{align}
 \begin{align}
     \sum_{i \in I} \sum_{j \in J} f_{uv}^{ij}  \leq q_{uv}\; \quad \forall (u,v) \in E
     \label{c5b}
 \end{align}
  \noindent\textbf{Flow Constraints: }
 \begin{align}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad a_i x_{ii} + \sum_{v\in V: (i,v) \in E}\sum_{j \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1b}
\end{align}

\begin{equation}
    \begin{aligned}
        &\quad \sum_{v \in V: (v,u) \in E}f^{ij}_{vu} - \sum_{v \in V: (u,v) \in E}f^{ij}_{uv} = a_i x_{iu} \; \\% a_i x_{iu}\; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i%, u \neq j
    \end{aligned}
    \label{flow2b}
\end{equation}

%%%%%%%%%%%%%%%%%%
\noindent\textbf{Domain Constraints: }
\begin{align}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1b}
\end{align}
\begin{align}
    \quad  x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
    \label{dom2b}
\end{align}
\begin{align}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall (u,v) \in E, i \in I, j \in J
    \label{dom3b}
\end{align}

The objective function minimizes the total cost comprised of two terms; the first one represents the cost of installing and operating a gateway at location $j$, aggregated over the total number of gateways used. %The second term accounts for the demand allocation cost, where $c_{ij}$ denotes the cost of supplying by gateway j the fraction $x_{ij}$  of the demand $a_i$ originating at $i$. 
The second term corresponds to the transport/connection cost from the demand originating at $i$ to its assigned gateway $j$, aggregated for all demands.

Constraints set \eqref{c1b} assures that traffic demands are supported by the selected gateways. Feasibility constraints set \eqref{c2b} makes sure that demands are only served by open gateways.
% while according to \ref{c3b} the amount of traffic from the demand originating at $i$ assigned to gateway $j$ passing through the link $(u,v)$ cannot exceed the requested traffic demand $a_i$. Constraints \eqref{c4b} and \eqref{c5b} state the capacity constraints for the gateways and the links.
Constraints \eqref{flow1b} and \eqref{flow2b} enforce the flow conservation.
The domains of $y_i$, $x_{ij}$ and $f_{uv}^{ij}$ variables are defined in constraints \eqref{dom1b}, \eqref{dom2b}, \eqref{dom3b}, respectively. 

In the aforementioned formulation, %considering the constraints \eqref{c3b},   %we can alleviate %the constraints set \ref{c4b} if we do not consider any other constrained resource (e.g., maximum CPU load) on the potential gateways, as well as 
%the $2^{nd}$ term of the objective function since we do not consider any demand allocation cost.
 we can express the set of $x_{ij}$ variables, utilizing the corresponding last-hop flow variables:

\begin{equation}
    x_{ij} = \frac{\sum_{u \in V}{f^{ij}_{uj}}}{a_i},\; \quad \forall i \in I, j \in J
    \label{aux}
\end{equation}

We can replace the set of $x_{ij}$ variables as in \eqref{aux}. The new MILP model for JSGPR is presented in the next subsection.
% Furthermore in order to meet the end-to-end delay requirements for each demand point $i$ we will impose a new constraint exploiting the corresponding flow variables: 

% \begin{equation}
%     \quad \sum_{j \in J}\sum_{uv \in L}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
%     \label{newdelgar}
% \end{equation}
% Where $d_max$ is the maximum of tolerable average end-to-end delay by a terrestrial node and $d_{uv}$ is the value of the propagation delay induced by the terrestrial link $(u,v)$. The equation \eqref{newdelgar} implies that the average experienced delay by node $i$'s traffic over all the flows originated at $i$, does not exceed the imposed upper bound. The next subsection entails the new derived MILP model.

\subsection{JSGPR MILP Formulation II}
% In order to formulate the JSGPR problem as a MILP we consider 
% \begin{itemize}
%     \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
%     \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the traffic rate passing through the link $(u,v)$ corresponding to flow $i\rightarrow j$.
% \end{itemize}

The new MILP formulation is as follows:
%as a mixed integer-linear program (MILP) which will follow. 

% \vspace{2mm}
% \noindent\textbf{Objective function:}
% \begin{equation}
%     \textbf{Minimize} \quad \sum_{i\in V}{x_i} + 1/N\sum_{n \in V}\sum_{ij \in E}{z_n^{ij}d_{ij}}
% \end{equation}

% \begin{equation}
%     \sum_{i \in V}{y_{ij}} = 1,\; \quad \forall j \in V
% \end{equation}

% \begin{equation}
%     y_{ij}\leq x_i, \; \quad \forall i,j \in V
% \end{equation}

% \begin{equation}
%     \sum_{iv \in E}{z^{iv}_{j}} - \sum_{ui \in E}{z^{ui}_{j}}  = y_{ij}. \; \quad \forall i,j \in V
% \end{equation}

% \vspace{2mm}
% \noindent\textbf{Objective: }
% \begin{equation}
%     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
% \end{equation}


% \noindent\textbf{Demand Guarantee Constraints: }
% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
% \end{equation}

% \noindent\textbf{Feasibility Guarantee Constraints: }
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}a_ix_{ij} \leq b_jy_j,\; \quad \forall j \in J 
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq a_ix_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Link Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
% \end{equation}

% \noindent\textbf{Flow Constraints: }
% \begin{equation}
%     \quad a_ix_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + a_ix_{iu}, \; \\ 
%         & \quad \forall i \in I, u \in V,  u \neq i
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

% \begin{equation}
%     \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
% \end{equation}

% \begin{equation}
%     \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
% \end{equation}


% \newpage

\vspace{2mm}
% \noindent\textbf{Objective: }
\begin{equation}
    \textbf{Minimize} \quad%(1-\phi)%
    \sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{(u,v) \in E}c_{uv}f^{ij}_{uv} \;
    \label{obj}
    %     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j}\;
    % \label{obj}
\end{equation}


\noindent\textbf{Demand  Constraints: }
\begin{equation}
    \quad\sum_{j \in J}\sum_{u \in V} f^{ij}_{uj} = a_i,\; \quad \forall i \in I 
    \label{demgar}
\end{equation}

\noindent\textbf{Feasibility  Constraints: }
\begin{equation}
    \quad \sum_{u \in V} f^{ij}_{uj} \leq y_j a_i,\; \quad \forall i \in I, \forall j \in J 
    \label{leq}
\end{equation}

% \noindent\textbf{Delay Guarantee Constraints:}
% \begin{equation}
%     \quad \sum_{j \in J}\sum_{uv \in L}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
%     \label{delgar}
% \end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq b_jy_j,\; \quad \forall j \in J 
%     \label{cap}
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq \sum_{u \in V} f^{ij}_{uj},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
%     \label{maxflow}
% \end{equation}

\noindent\textbf{Capacity Constraints: }
  \begin{equation}
     \sum_{i\in I}\sum_{u\in V}{f^{ij}_{uj}} \leq q_j y_j,\; \quad \forall j \in J
     \label{c4b2}
 \end{equation}
\begin{equation}
    \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall (u,v) \in E
    \label{linkcap}
\end{equation}

\noindent\textbf{Flow Constraints: }
\begin{equation}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
         \sum_{u \in V: (u,i) \in E}{f^{ii}_{ui}} + \sum_{v\in V: (i,v) \in E}\sum_{j\neq i \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1}
\end{equation}

\begin{equation}
    \begin{aligned}
         %&\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + \sum_{u \in V} f^{iu}_{uu}, \; \\ 
        % & \quad \forall i \in I, u \in V,  u \neq i
        %&\quad \sum_{v \in V: (u,v) \in L}f^{ij}_{vu} - \sum_{v \in V: (u,v) \in L}f^{ij}_{uv} = a_i x_{iu} \; \\ 
        &\quad \sum_{v \in V: (u,v) \in E}f^{ij}_{vu} - \sum_{v \in V: (u,v) \in E}f^{ij}_{uv} = \sum_{u \in V}{f^{iu}_{uu}} \; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i%, u \neq j
    \end{aligned}
    \label{flow2}
\end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

\noindent\textbf{Domain Constraints: }
\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1}
\end{equation}

\begin{equation}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall (u,v) \in E, i \in I, j \in J
    \label{dom2}
\end{equation}

\vspace{2mm}


% The first term of the objective function \eqref{obj} is the cost associated with the deployment of the gateways while the second term is the average end-to-end delay of all the flows which traverse the network.  We aim at minimizing the objective function seeking a trade-off between the two terms. The trade-off factor in the objective function is denoted by $\phi$.

% //////////?Comment?/////

%Newly commented
% The objective function \eqref{obj} is the total cost of the process, consisting of the gateway deployment cost and the bandwidth cost
% Constraints \eqref{demgar} are to ensure that the traffic demand for each node is satisfied using one or multiple gateways. Constraints \eqref{leq} allow for the formation of the flow $i\rightarrow j$ only if a gateway is placed at node $j$, while constraints \eqref{delgar} will guarantee that the average end-to-end delay for each demand point will not exceed a pre-defined upper bound $d_{max}$.

% , while constraints \eqref{cap} ensure that the load on each gateway is less than the capacity of the gateway (i.e. less than the capacity of the gateway-satellite node.)
% By constraints \eqref{maxflow}, the rate that each link $(u,v)$ allocates to flow $i\rightarrow j$ is at most equal to the part of the demand of node $i$ which gateway $j$ is responsible for.
%newly commented
% Constraints \eqref{linkcap} make sure that the resources allocated by each link does not exceed the capacity of that link. Constraints \eqref{flow1} and \eqref{flow2}  enforce the flow conservation; i.e. the inbound traffic to a switch must be equal to its outbound traffic. Finally, the  constraints \eqref{dom1}, and \eqref{dom2} express the domain requirements for the variables $\textbf{y}$, and $\textbf{f}$ respectively.
% We also define another notation which does not show up in the problem setup but becomes useful for further discussions. Let $\textbf{x}$ be a set of $x_{ij}$ variables which represent the portion of the traffic originated by node $i$ which is going to be gatewayed to the satellite through gateway $j$. More precisely we write: 
% \begin{equation}
%     x_{ij} = \frac{\sum_{u \in V}{f^{ij}_{uj}}}{a_i}
%     \label{aux}
% \end{equation}
% Where $0\leq x_{ij}\leq1$. Utilizing \eqref{aux}, a few of the constraints in the above-mentioned minimization problem, including \eqref{demgar}, and \eqref{leq}, could be written in the somewhat more intuitive following form:

% % and \eqref{maxflow}, 

% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
%     \label{aux1}
% \end{equation}
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J
%     \label{aux2}
% \end{equation}
% % \begin{equation}
% %     \quad f^{ij}_{uv} \leq a_i x_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% %     \label{aux3}
% % \end{equation}
% With this alternative notation, the formulated problem very much looks like a variant of the facility location problem formulated in \cite{Bell}; Utilizing the flow variables in the described fashion allows for path splitting which improves the flexibility of the network, and the efficiency of link usage.

Where $\phi = \frac{1}{(\sum_{i\in I}{a_i})}$ is the normalization factor between the two terms of the objective function.
Additionally, in order to meet the average delay requirement for each demand point $i$ we will impose a new constraint exploiting the corresponding flow variables: 

\begin{equation}
    \quad \sum_{j \in J}\sum_{(u,v) \in E}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
    \label{newdelgar}
\end{equation}
where $d_{max}$ is the maximum allowed average delay for each terrestrial node. We note that we have ignored the delay of the terrestrial-satellite link in the above calculation, since it is a constant term as explained in section \ref{sec:desc}.
%The equation \eqref{newdelgar} implies that the average experienced delay by node $i$'s traffic over all the flows originated at $i$, does not exceed the imposed upper bound.


% %TABLE///////////////////%

% \begin{table}[h]
% \centering
% \label{table}
% \begin{center}
% {
% \begin{tabularx}{\textwidth}{|c|X|}

% \hline
% Variables & Description\\
% \hline
% %$q_l[i]$ & Location of the UAV l at timeslot i\\
% $y_j$ & Binary variable determining whether or not a gateway is placed at node $j$. \\
% % $ $ & kjh\\
% $x_{ij}$ & Continuous variable in [0, 1] determining the portion of demanded traffic for node i, which is routed through node j. \\
% $f_{uv}^{ij}$ & The flow passing through the link $(u,v)$ corresponding to node $i$ destined at gateway j.\\
% \hline
% Parameters & Description\\
% \hline
% $a_i$ & Overall traffic generated at node $i$ \\
% $c_j$ & The cost of placing a gateway at node $j$\\
% $d_{uv}$ & The delay corresponding to routing packets through the link $(u,v)$\\
% $q_{uv}$, &Flow capacity of the link $(u,v)$ \\
% %$\rho_0$ & Channel power gain at the reference distance of 1m\\
% %$\gamma_{min}$ & Minimum received SNR for a successful transmission\\
% %$\sigma_n^2$ & Thermal noise power\\
% %$E$ & Transmission power of the nodes\\
% %$d_{min}$ & minimum allowed distance between two UAVs\\
% \hline
% \end{tabularx}}
% \end{center}
% \caption{Variables and Parameters Description}
% \end{table}


\subsection{JSGPR-LB MILP Formulation}

 In the aforementioned specification, the assigned load to a gateway is solely bounded by the capacity constraints \eqref{c4b2} and \eqref{linkcap}. We define a new single decision variable $l_{max}$ to represent the maximum traffic assigned to a gateway, common for all the selected gateways. We add $l_{max}$ as an additional term to the objective function. The new objective function is described in \eqref{objlm}:
 %i.e. by the minimum of the aggregated capacity of the incoming links to the gateway, and the capacity of the terrestrial-satellite link.% Moreover, if the capacity of the terrestrial-satellite link is high enough, constraint \eqref{c4b2} can be omitted. We call this non-capacitated variant of our algorithm, $JSGPR-NC$. 
 %In order to optimize the load among selected gateways we multiply the summation representing the inbound traffic towards the terrestrial-satellite link of the selected gateways with the utilization of the link for each respective gateway as described in \ref{objlm}, aggregated over the gateways. The summation has a third term in the objective, excluding the corresponding cost from the second term.  %In order to minimize the forwarding latency, and balance the load on the gateways, we wish to minimize the value of $l_{max}$\cite{manet}, \cite{lb}. Hence, we will add $l_{max}$ as an additional term to the objective function. The new objective function will look like:

\begin{align}
    % \textbf{Minimize} \quad(1-\phi)\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
    % \label{obj}
    %\textbf{Minimize} \sum_{j \in J} c_j y_{j}+ \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L,v \neq j} c_{uv}f^{ij}_{uv}+ \nonumber \\ 
   % \phi\sum_{i \in I}\sum_{j \in J}\sum_{uj \in L} c_{uj}(1-\frac{r_{uj}}{g_j})f^{ij}_{uj}\;% + \alpha  l_{max}\;
       \textbf{Minimize} \quad(\sum_{j \in J}c_jy_{j}+\phi\sum_{i \in I}\sum_{j \in J}\sum_{(u,v) \in E}c_{uv}f^{ij}_{uv}) + \alpha l_{max}\;
    \label{objlm}
\end{align}
where $\alpha$ is a constant factor determining the balance between the two terms of the objective function.  
Also, we change  constraints \eqref{c4b2} as following:
\begin{equation}
         \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq l_{max}\; \quad \forall j \in J 
\end{equation}
where $l_{max} \leq q_j \quad \forall j \in J$. We will call this last model, $JSGPR-LB$. The resulted optimization problem aims to balance the load of the gateways in conjunction with the cost of the gateway deployment \cite{manet}, \cite{lb}. 

\subsection{LP Relaxation and Approximation Algorithm}

Since the MILP model is known to be NP-hard, the problem is intractable for larger scale networks \cite{Bell}. For the aforementioned JSGPR and JSGPR-LB MILP formulations, the optimal fractional solution is computed for the problem via linear programming relaxation. The relaxed problem can be solved by any suitable linear programming method, in polynomial time. A rounding technique is applied, similar to \cite{torkzaban2019trust} to obtain the integer solution of the MIP problem. The resulting multi-commodity flow allocation problem is solved to identify the routing paths. 
% \begin{equation}
%     % \textbf{Minimize} \quad(1-\phi)\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
%     % \label{obj}
%         \textbf{Minimize} \quad(\sum_{j \in J}c_jy_{j}+\phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}) + \alpha l_{max}\;
%     \label{objlm}
% \end{equation}


% Moreover, if the capacity of the terrestrial-satellite link is high enough, constraint \eqref{c4b2} can be omitted. Instead, to ensure that the traffic assigned to each gateway does not exceed $l_{max}$, we add the following set of constraints to our model:

% \begin{equation}
%          \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq l_{max}\; \quad \forall j \in J 
% \end{equation}



==> Satellite Gateway Placement Problem/introduction1.tex <==
\section{Introduction}
Over the past years, the integration of satellite communications with current and emerging terrestrial networks (e.g., 5G mobile networks) is gaining attention, given the growing data traffic volume which is predicted to increase by over 10,000 times in the next 20 years \cite{8438267}. The trend is also supported by national directives and initiatives to support broadband connectivity in rural and remote areas, as it is considered a crucial factor for economic growth. Due to their large footprint, satellites can complement and extend terrestrial networks, both in densely populated areas and in rural zones, and provide reliable mission critical services. Standardization bodies as 3GPP, ETSI \cite{doi:10.1002/sat.1292} and ITU \cite{8438267} also recognize and promote integrated and/or hybrid satellite and terrestrial networks.

The integrated satellite-terrestrial networks (ISTNs) can be a cornerstone to the realization of a heterogeneous global system to enhance the end-user experience \cite{artiga2016terrestrial}. An ISTN, as depicted in Fig.~\ref{fig:map}, is composed of satellites organized in a constellation that support routing, adaptive access control, and spot-beam management \cite{vasavada2016architectures}, whereas the  terrestrial optical network consists of ground stations (gateways), switches, and servers. %Similar to \cite{guo19} the links of the satellite network are inter-satellite links (ISLs), and the links of the terrestrial network are optical fiber for higher bandwidth.  
Delay-sensitive data services are more suitable to transport in the low earth orbit (LEO) satellite networks, which provide inherent advantages in power consumption, pole coverage, latency, and lower cost compared with the geostationary earth orbit (GEO) satellite networks and the medium earth orbit (MEO) satellite networks \cite{guo19}. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{results/ICC2020/SGP2.jpg}
\caption{Example of an integrated satellite-terrestrial network.}
\label{fig:map}
\end{center}
\end{figure}


However, there are multiple challenges associated with the ISTNs. Satellite networks and terrestrial networks are widely heterogeneous, supported by distinct control and management frameworks, thus their integration to date was based on proprietary and custom solutions.  Additionally, in the integrated network, as there are multiple available paths along which data traffic can be routed, optimized path-selection is important to satisfy the Quality of Service (QoS) requirements of the traffic flows and improve the utilization of network resources \cite{jia2016broadband}. Existing satellite networks employ a decentralized management architecture, scheduled link allocation and static routing strategies, which make it difficult to support flexible traffic scheduling adapting to the changes in traffic demands \cite{service}. Complex handover mechanisms should be in place at the gateway nodes, while their high-power consumption requirements need to be also taken into consideration.

Nowadays the inclusion of plug-and-play SatCom solutions are investigated, primarily in the context of 5G. Exploiting software-defined networking (SDN)\cite{zhang2017energy} and network function virtualization (NFV), ISTNs can be programmed and network behavior can be centrally controlled using open APIs, thus supporting a more agile integration of terrestrial (wired and wireless) and satellite domains interworking with each other to deliver end-to-end services. Based on the extra degrees of freedom in ISTN deployment, brought forth by the softwarization and programmability of the network, the satellite gateway placement problem is of paramount importance for the space-ground integrated network. The problem entails the selection of an optimal subset of the terrestrial nodes for hosting the satellite gateways while satisfying a group of design requirements. Various strategic objectives can be pursued when deciding the optimal placement of the satellite gateways including but not limited to cost reduction, latency minimization, reliability assurance, etc. \cite{GW}, \cite{GWC}, \cite{taghlid}.


%The integration of satellites with terrestrial networks is gaining more attention, given the daily-increasing demand for data traffic. Offloading the unsettled demand, improving the congestion conditions in congested networks, extending the coverage, load balancing, higher trustworthiness and availability, etc., can be achieved by such an integration. Moreover, satellites can be used as the primary means for communications over rural areas, or any other environment where a robust terrestrial infrastructure setup is not possible. More importantly, satellites can be very well applied to the key $5G$ scenarios, since (i) they are capable of supporting a very large data rate (i.e., Gigabits per second), for enhanced mobile broadband communications, (ii) they can satisfy the daily increasing need for trust and availability, by supporting ultra-reliable communications , (iii) they support massive machine-to-machine communications, (iv) they can help $5G$ to meet its latency requirements by delivering the commonly accessed data to mobile base stations.

%However, there are multiple challenges associated with the integration of satellites and terrestrial networks; (i) The resulting ISTN, requires  new routing schemes which are capable of exchanging data between the ground and the space nodes while satisfying the QoS requirements \cite{GW}. (ii) The need for communications between the ground nodes and the satellites introduces higher power consumption requirements which needs to be taken care of prior to the integration. (iii) The network controllers need to perform more complex tasks, including the hand-off procedure between space nodes \cite{GWC}. (iv) The excessive delay between the ground and the space nodes becomes prohibitive in several delay-critical use-cases, which reveals the need for complementary technologies to satisfy the delay requirements. 

%With the emergence of software-defined networking (SDN) and network function virtualization (NFV), besides the significant reduction in capital and operational expenses, the increased complexity of the ISTNs can be managed in a centralized manner which allows for a more agile integration, flexible and dynamic traffic scheduling, and user-specified services \cite{service}. On this ground, to overcome the issues related to communications between the ground and the space nodes, the placement problem of the satellite gateways becomes of a paramount importance \cite{GW}. The problem entails the selection of an optimal subset of the terrestrial nodes for hosting the satellite gateways while satisfying a group of design requirements. Various strategic objectives can be pursued when deciding the optimal placement of the satellite gateways including but not limited to cost reduction, latency minimization, reliability assurance, etc. \cite{GW}, \cite{GWC}, \cite{taghlid}. 

 In this paper, we propose a method for the cost-optimal deployment of satellite gateways on the terrestrial nodes. Particularly, we aim to minimize the overall cost of gateway deployment and traffic routing, while satisfying latency requirements. To this end, we formulate the problem as a mixed-integer linear program (MILP), with latency bounds as hard constraints. We derive an approximation method from our MILP model to significantly reduce the time-complexity of the solution, at the expense of sub-optimal gateway placements, and investigate the corresponding trade-off. Furthermore, in order to reduce latency and processing power at the gateways, we impose a (varying) upper bound on the load that can be supported by each gateway.
 
 
% to decrease the load on the gateways in order to reduce the forwarding latency and the demand for processing power at nodes, we impose a varying upper bound on the traffic load at each gateway and wish to minimize that bound.
%In other words, we strike a balance between the time complexity of the solving process and the accuracy of the resulting solution.
It is important to note that, traffic routing and facility placement
are usually solved as different problems, but assigning
a demand point to a facility without considering the other
demand points might not be realistic [9]. Given the significant
interrelation of the two problems we develop and solve a single
aggregated model instead of solving the two problems in a
sequential manner.

The remainder of the paper is organized as follows. Section~\ref{sec:desc} describes the problem and the network model. In Section~\ref{sec:problem} we introduce the MILP formulation and its LP-based approximation followed by a variant of our model with load minimization. We present our evaluation results in section \ref{sec:evaluation}, and provide the overview of the related works in section \ref{sec:relatedwork}. Finally, in Section \ref{sec:conclusions}, we highlight our conclusions and discuss the directions for our 
future work.

==> Satellite Gateway Placement Problem/problem_description.tex <==
\section{Network Model and Problem Description} 
\label{sec:desc}
The ISTN network under our study is depicted in Fig. \ref{fig:map}.We model the terrestrial network as an undirected $G = (V, E)$ graph where $(u,v) \in E $ if there is a link between the nodes $u,v \in V$. Let $J\subseteq V $ be the set of all potential nodes for gateway placement and $I\subseteq V$ be the set of all demand points. We note that the sets $I$ and $J$ are not necessarily disjoint. A typical substrate node $v \in V$ may satisfy one or more of the following statements: (i) node $v$ is a gateway to the satellite, (ii) node $v$ is an initial demand point of the terrestrial network, (iii) node $v$ relays the traffic of other nodes, to one or more of the gateways. The ideal solution will introduce a set of terrestrial nodes for gateway placement which result in the cheapest deployment \& routing, together with the corresponding routes from all the demand points to the satellite, while satisfying the design constraints. 


%We consider an undirected $G = (V, E)$ graph to represent the studied terrestrial network where $(u,v) \in E $ if there is a link between the nodes $u,v \in V$. We consider a GEO satellite to be integrated with the terrestrial network. Let $J\subseteq V $ be the set of all candidates for gateway placement and $I\subseteq V$ be the set of all demand points. We note that the sets $I$ and $J$ are not necessarily disjoint. A typical substrate node $v \in V$ may satisfy one or more of the following statements. (i) Node $v$ is a gateway to the satellite., (ii) Node $v$ is an initial demand point of the terrestrial network., (iii) Node $v$ relays the traffic of other nodes, to one or more of the gateways. The ideal solution will introduce the cheapest set of terrestrial nodes as the ideal placement for the gateways, and the routes from all the demand points to the satellite, while satisfying the design constraints. 
%We note that, for each demand point


% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.45\textwidth]{figures/scene2.jpeg}
% \caption{Example of an integrated satellite-terrestrial network.}
% \label{fig:map}
% \end{center}
% \end{figure}
Regarding the delay of the network we consider only propagation delay. %and forwarding/processing delay. 
The propagation delay of a path in the network is the sum of the propagation delays over its constituting links. A GEO satellite is considered in the particular system model \cite{GW}. Let $d_{uv}$ represent the contribution of the terrestrial link $(u,v)$ to the propagation delay of a path which contains that link. The propagation delay from a gateway to the satellite is constant \cite{GWC}. Moreover, we consider multi-path routing for the traffic demands. Therefore, we define a flow $i\rightarrow j$ as the fraction of the traffic originated at node $i \in I$, routed to the satellite through gateway $j \in J$. 

%The delay is mostly determined by the traffic load on each gateway. 
Once all the flows corresponding to node $i$ are determined, all the routing paths from node $i$ to the satellites are defined. Let $c_j$ denote the cost associated with deploying a satellite gateway at node $j$ and $c_{uv}$ the bandwidth unit cost for each link $(u,v)$. We also define $a_i$ as the traffic demand rate of node $i$ which is to be served by the satellite. The capacity of each link $(u,v)$ is denoted by $q_{uv}$ while the capacity of the gateway-satellite link is $q_j$ for gateway $j$. Table \ref{paramv} summarizes all the notations used for the parameters and variables throughout the paper.

%table of notations
\begin{table*}[ht]
\centering
\begin{center}
\scalebox{0.9}{
\begin{tabular}{|c|c|}
\hline
Variables & Description\\
\hline
$y_j$ & The binary decision variable of gateway placement at node $j$\\
$x_{ij}$ & The fraction of traffic demand originating at $i$ passing through gateway $j$\\
$f_{uv}^{ij}$ & The amount of traffic originating at $i$ assigned to gateway $j$ passing through the link $(u,v)$\\
\hline
Parameters & Description\\
\hline
$G= (V,E)$ & Terrestrial network graph\\
$J$ & The set of potential nodes for gateway placement \\
$I$ & The set of demand points\\
$c_j$ & The cost associated with deploying a satellite gateway at node $j$\\
$c_{uv}$ & Bandwidth unit cost for link $(u,v)$\\
$a_i$ & Traffic demand rate of node $i$\\
$q_{uv}$ & Capacity of link $(u,v)$\\
$q_j$ & Capacity of gateway-satellite link for gateway $j$\\
\hline
\end{tabular}}
\caption{System model parameters and variables}
\label{paramv}
\end{center}
\end{table*}

%%end of notation table

Since the propagation latency is usually the dominant factor in determining the network delay \cite{taghlid}, we first develop a joint satellite gateway placement and routing (JSGPR) MILP formulation to minimize the cumulative gateway placement cost with hard constraints on the average %end-to-end
propagation delay for the traffic of each demand point.

%The demand of node $i$ may be satisfied by multiple flows $\{i\rightarrow j: j \in V\}$, and each flow $i\rightarrow j$ might exploit multiple different paths with different corresponding delays between the nodes $i$ and $j$. This should be taken into account in the calculation of the average delay for each demand point. The forwarding delay is mostly determined by the traffic load on each gateway. We also note that once all the flows corresponding to node $i$ is determined, all the routing paths from node $i$ to the satellites are uniquely determined. 

Following that, we will derive a variant of JSGPR with load balancing (JSGPR-LB) which aims at mutually optimizing the overall cost and the load assigned to all the deployed gateways. Finally, we use an LP-based approximation approach to reduce the time-complexity of the proposed scheme at the cost of a sub-optimal gateway placement.
% JSGPR entails the placement of a set of gateways with a maximum size of $|J|$, on the terrestrial nodes to facilitate the ground-space communications, as well as deciding the routes between the terrestrial switches and the satellite, while minimizing the overall gateway placement cost and satisfying the hard constraints on the end-to-end delay requirements. Within the same context, JSGPR-LM wishes to minimize the maximum traffic which may be assigned to a gateway after the placement. 


% It is important to note that, traffic routing and facility placement are usually solved as different problems, but assigning a demand point to a facility without considering the other demand points might not be realistic\cite{Bell}. Given the significant interrelation of the two problems we develop and solve a single aggregated model Instead of solving the two problems in a sequential manner.
% We note that, there is a subset of nodes which are used as relays and might not be the source of any original traffic. 

% We introduce a set of $\textbf{x} = x_1^n$ variables to represent the assignment of gateways, where $x_i = 1$ if and only if a gateway is going to be placed on node $i$. The $\textbf{y} = y_{11}^{nn}$ set of variables denotes the assignment of terrestrial switches to the satellite gateways. Particularly, $y_{ij} = 1$ if and only if, node $i$ is the chosen gateway for switch $j$. 

==> Satellite Gateway Placement Problem/related_work.tex <==
\section{Related Work}
\label{sec:relatedwork}
 Although the gateway placement problem over a general network is very-well studied, the satellite gateway placement problem on an ISTN is fairly new. 
 For sensor \cite{bzoor}, vehicular\cite{mezza}, wireless mesh \cite{gorbe} and MANETs \cite{manet}, different approaches have been proposed with different optimization objectives such as load balancing \cite{lb}, latency minimization \cite{delay}, reliability maximization \cite{rel}, etc. 
 
 
 The recent works on ISTNs , mostly focus on optimizing the average network latency\cite{GW} or reliability\cite{GWC}, \cite{capac}, \cite{taghlid}, \cite{same}. In \cite{GW}, the authors propose a particle swarm-based optimization approximation (PSOA) approach for mimizing the average network latency and benchmark it against an optimal brute force algorithm (OBFA) to show the imporvement in the time complexity. In \cite{GWC}, a hybrid simulated annealing and clustering algorithm (SACA) is used to provide near optimal solution for the joint SDN controller and satellite gateway placement with the objective of network reliability maximization.  For the same purpose as \cite{GWC}, authors in \cite{taghlid}, provide a simulated annealing  partion-based k-means (SAPKM) approach and compare the advantages and weaknesses of their approach with that of \cite{GWC}. In \cite{capac}, the authors consider the satellite link capacity as a limiting constraint and solve the placement problem to maximize the reliability. 
 
 There is another line of research which aims to place the satellite gateways on the aerial platforms. More precisely in \cite{cross}, a new aerial layer is added in between the terrestrial and the satellite layer which relays the traffic between the satellite and the terrestrial nodes. The authors have used a greedy optimization approach to make the gateway selection.
 
 Although the above approaches provide a great insight into the satellite gateway placement problem, they assume the number of gateways is known prior to design. Secondly, none of the above studies investigates the traffic routes from the terrestrial switches to the satellite, whereas we propose the joint optimization of satellite gateway placement together with the corresponding traffic routing for ISTNs. %To the best of our knowledge, we are the first to study the problem of satellite gateway placement together with the corresponding traffic routing problem. 

==> formulation_old.tex <==
\section{Problem Formulation}
\label{sec:problem}
\subsection{JSGPR MILP Formulation}
In order to formulate the JSGPR problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the traffic rate passing through the link $(u,v)$ corresponding to flow $i\rightarrow j$.
\end{itemize}

The MILP formulation is as follows:
%as a mixed integer-linear program (MILP) which will follow. 

% \vspace{2mm}
% \noindent\textbf{Objective function:}
% \begin{equation}
%     \textbf{Minimize} \quad \sum_{i\in V}{x_i} + 1/N\sum_{n \in V}\sum_{ij \in E}{z_n^{ij}d_{ij}}
% \end{equation}

% \begin{equation}
%     \sum_{i \in V}{y_{ij}} = 1,\; \quad \forall j \in V
% \end{equation}

% \begin{equation}
%     y_{ij}\leq x_i, \; \quad \forall i,j \in V
% \end{equation}

% \begin{equation}
%     \sum_{iv \in E}{z^{iv}_{j}} - \sum_{ui \in E}{z^{ui}_{j}}  = y_{ij}. \; \quad \forall i,j \in V
% \end{equation}

% \vspace{2mm}
% \noindent\textbf{Objective: }
% \begin{equation}
%     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
% \end{equation}


% \noindent\textbf{Demand Guarantee Constraints: }
% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
% \end{equation}

% \noindent\textbf{Feasibility Guarantee Constraints: }
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}a_ix_{ij} \leq b_jy_j,\; \quad \forall j \in J 
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq a_ix_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Link Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
% \end{equation}

% \noindent\textbf{Flow Constraints: }
% \begin{equation}
%     \quad a_ix_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + a_ix_{iu}, \; \\ 
%         & \quad \forall i \in I, u \in V,  u \neq i
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

% \begin{equation}
%     \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
% \end{equation}

% \begin{equation}
%     \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
% \end{equation}


% \newpage

\vspace{2mm}
\noindent\textbf{Objective: }
\begin{equation}
    \textbf{Minimize} \quad%(1-\phi)%
    \sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv} \;
    \label{obj}
    %     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j}\;
    % \label{obj}
\end{equation}


\noindent\textbf{Demand Guarantee Constraints: }
\begin{equation}
    \quad\sum_{j \in J}\sum_{u \in V} f^{ij}_{uj} = a_i,\; \quad \forall i \in I 
    \label{demgar}
\end{equation}

\noindent\textbf{Feasibility Guarantee Constraints: }
\begin{equation}
    \quad \sum_{u \in V} f^{ij}_{uj} \leq y_j a_i,\; \quad \forall i \in I, \forall j \in J 
    \label{leq}
\end{equation}

\noindent\textbf{Delay Guarantee Constraints:}
\begin{equation}
    \quad \sum_{j \in J}\sum_{uv \in L}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
    \label{delgar}
\end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq b_jy_j,\; \quad \forall j \in J 
%     \label{cap}
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq \sum_{u \in V} f^{ij}_{uj},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
%     \label{maxflow}
% \end{equation}

\noindent\textbf{Link Capacity Constraints: }
\begin{equation}
    \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
    \label{linkcap}
\end{equation}

\noindent\textbf{Flow Constraints: }
\begin{equation}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad f^{ii}_{ii} + \sum_{v\in V: iv \in L}\sum_{j\neq i \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1}
\end{equation}

\begin{equation}
    \begin{aligned}
        % &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + \sum_{u \in V} f^{iu}_{uu}, \; \\ 
        % & \quad \forall i \in I, u \in V,  u \neq i
        &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} \; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i
    \end{aligned}
    \label{flow2}
\end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1}
\end{equation}

\begin{equation}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
    \label{dom2}
\end{equation}

\vspace{2mm}
% The first term of the objective function \eqref{obj} is the cost associated with the deployment of the gateways while the second term is the average end-to-end delay of all the flows which traverse the network.  We aim at minimizing the objective function seeking a trade-off between the two terms. The trade-off factor in the objective function is denoted by $\phi$.
The objective function \eqref{obj} is the total cost of the process, consisting of the gateway deployment cost and the bandwidth cost
Constraints \eqref{demgar} are to ensure that the traffic demand for each node is satisfied using one or multiple gateways. Constraints \eqref{leq} allow for the formation of the flow $i\rightarrow j$ only if a gateway is placed at node $j$, while constraints \eqref{delgar} will guarantee that the average end-to-end delay for each demand point will not exceed a pre-defined upper bound $d_{max}$.
% , while constraints \eqref{cap} ensure that the load on each gateway is less than the capacity of the gateway (i.e. less than the capacity of the gateway-satellite node.)
% By constraints \eqref{maxflow}, the rate that each link $(u,v)$ allocates to flow $i\rightarrow j$ is at most equal to the part of the demand of node $i$ which gateway $j$ is responsible for. 
Constraints \eqref{linkcap} make sure that the resources allocated by each link does not exceed the capacity of that link. Constraints \eqref{flow1} and \eqref{flow2}  enforce the flow conservation; i.e. the inbound traffic to a switch must be equal to its outbound traffic. Finally, the  constraints \eqref{dom1}, and \eqref{dom2} express the domain requirements for the variables $\textbf{y}$, and $\textbf{f}$ respectively.

% We also define another notation which does not show up in the problem setup but becomes useful for further discussions. Let $\textbf{x}$ be a set of $x_{ij}$ variables which represent the portion of the traffic originated by node $i$ which is going to be gatewayed to the satellite through gateway $j$. More precisely we write: 
% \begin{equation}
%     x_{ij} = \frac{\sum_{u \in V}{f^{ij}_{uj}}}{a_i}
%     \label{aux}
% \end{equation}
% Where $0\leq x_{ij}\leq1$. Utilizing \eqref{aux}, a few of the constraints in the above-mentioned minimization problem, including \eqref{demgar}, and \eqref{leq}, could be written in the somewhat more intuitive following form:

% % and \eqref{maxflow}, 

% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
%     \label{aux1}
% \end{equation}
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J
%     \label{aux2}
% \end{equation}
% % \begin{equation}
% %     \quad f^{ij}_{uv} \leq a_i x_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% %     \label{aux3}
% % \end{equation}

% With this alternative notation, the formulated problem very much looks like a variant of the facility location problem formulated in \cite{Bell}; Utilizing the flow variables in the described fashion allows for path splitting which improves the flexibility of the network, and the efficiency of link usage.

Since the MILP is known to be NP-hard, the proposed formulation is intractable for larger scale networks. Next we derive an LP model to strike a balance between the time-complexity of the optimization problem and the accuracy of the results.   


% %TABLE///////////////////%

% \begin{table}[h]
% \centering
% \label{table}
% \begin{center}
% {
% \begin{tabularx}{\textwidth}{|c|X|}

% \hline
% Variables & Description\\
% \hline
% %$q_l[i]$ & Location of the UAV l at timeslot i\\
% $y_j$ & Binary variable determining whether or not a gateway is placed at node $j$. \\
% % $ $ & kjh\\
% $x_{ij}$ & Continuous variable in [0, 1] determining the portion of demanded traffic for node i, which is routed through node j. \\
% $f_{uv}^{ij}$ & The flow passing through the link $(u,v)$ corresponding to node $i$ destined at gateway j.\\
% \hline
% Parameters & Description\\
% \hline
% $a_i$ & Overall traffic generated at node $i$ \\
% $c_j$ & The cost of placing a gateway at node $j$\\
% $d_{uv}$ & The delay corresponding to routing packets through the link $(u,v)$\\
% $q_{uv}$, &Flow capacity of the link $(u,v)$ \\
% %$\rho_0$ & Channel power gain at the reference distance of 1m\\
% %$\gamma_{min}$ & Minimum received SNR for a successful transmission\\
% %$\sigma_n^2$ & Thermal noise power\\
% %$E$ & Transmission power of the nodes\\
% %$d_{min}$ & minimum allowed distance between two UAVs\\
% \hline
% \end{tabularx}}
% \end{center}
% \caption{Variables and Parameters Description}
% \end{table}
\subsection{LP Relaxation and Rounding Algorithm}

The LP model is obtained from the original MILP formulation by relaxing the integrality of the binary $\textbf{y}$ variables. We replace the domain constraints \eqref{dom1} by the following ones:

\begin{equation}
    \quad y_{j} \in [0, 1],\; \quad \forall j \in J
    \label{domain1new}
\end{equation}

The rest of the model remains intact. The LP model can be solved within a polynomial effort, but does not necessarily leave us with a valid gateway placement. Therefore, inspired by \cite{torkzaban2019trust}, we use a deterministic rounding algorithm to derive binary values for the $\textbf{y}$  placement variables, with the cost of solution suboptimality. The rounding is pseudo-coded in \textbf{Algorithm-\ref{alg}}, and works as follows; In each iteration (Lines \ref{2}-\ref{11}), first an LP model is solved, then the value $y_j$ for each satellite gateway candidate is extracted as presented in the line \ref{6}. Then the candidate corresponding to the maximum  $y_j$ is chosen to be rounded to $1$ and added to the LP model (Lines \ref{6}-\ref{8}). Since the $y_j$ variables only show up in the right half-side of the $(\leq)$constraints, non of the constraints get violated by this choice. The algorithm terminates after all the dimensions of the solution are rounded (i.e. no fractional values show up in the solution of the LP model), or when the LP model becomes infeasible in which case the gateway placement is denied. After the placement of the gateways is determined, a multi-commodity flow (MCF) allocation algorithm is run to find out the corresponding flow variables. 

Since the integral part of the solution has at most $|J|$ dimensions, the $\textbf{Solve\_LP(..)}$ function will run at most $|J|$ times which results in a polynomial time-complexity as stated earlier.
% We also note that in the calculation of $\lambda_j$, the product of $y_j$ and the total load on $jth$ gateway candidate, i.e. $\sum_{i\in I}{a_ix_{ij}}$ is obtained instead of merely considering the relaxed $y_j$ placement variables. This way a gateway candidate that both has a high fractional placement value, and a high amount of assigned load, is preferred to be chosen in the final placement choice.  


\begin{algorithm}
\caption{LP Rounding}
\label{alg}
\begin{algorithmic}[1]


\REPEAT \label{1}
    \STATE $\{y_j, f^{ij}_{uv}\} \leftarrow \textbf{Solve\_LP(..)}$ \label{2}

    \STATE If solution exists \textit{Sol:= true}, Otherwise \textit{Sol:= false} \label{3}

    \STATE  $Y \leftarrow\{y_j |y_j \notin \{0, 1\} \}$ \label{4}
    
   \IF{$Y \neq 0$} \label{5} 
   % \STATE  $X_a \leftarrow\{x^i_u |x^i_u \in X  \land g_{i} <= r_{u} \}$

    %\IF{$X_a \neq 0$}
  %   \STATE $\{i_0, u_0\} \leftarrow argmax_{\{i \in V_f, u \in V_s\}} X_a $
    % \STATE $\Lambda := \{\lambda_j:=y_j*(\sum_{i\in I}{x_{ij}})|j \in J\}$ \label{new}
    \STATE $\{y_0\} \leftarrow \arg \max_{\{j \in J\}} Y $ \label{6}
    % \IF{$\{i_0, u_0\}$ exists} \label{7}
    \STATE \textbf{Add LP Constraint $y_0=1$} \label{8}
    % \ELSE \label{9}
    % \STATE \textit{Sol=false} \label{10}
    \ENDIF \label{11}
    % \ENDIF \label{12}
\UNTIL $(Y=0) \lor(Sol =false)$ \label{13}   
%\UNTIL $(X=0) \lor (X_a=0) \lor   (Sol =false)$

\IF{$Sol= true$} \label{14}
\STATE $\{y_j, f^{ij}_{uv}\} \leftarrow \textbf{Solve\_MCF(..)}$ \label{15}

    \STATE If solution exists \textit{Sol:= true}, Otherwise \textit{Sol:= false} \label{16}
\ENDIF \label{26}
%    \IF{\textit{Sol:= true}} \label{17}
%\RETURN $\{x^i_u, f^{ij}_{uv}\}$ \{Accept the request\} \label{18}
%    \ELSE \label{19}
%    \STATE $\{\forall{x^i_u} :=0, \forall{f^{ij}_{uv}} :=0\}$ \label{20}
%   \RETURN $\{x^i_u, f^{ij}_{uv}\}$ \{Deny the request\} \label{21}
%    \ENDIF \label{22}
%\ELSE \label{23}
%\STATE $\{\forall{x^i_u} :=0, \forall{f^{ij}_{uv}} :=0\}$ \label{24}
%\RETURN $\{x^i_u, f^{ij}_{uv}\}$ \{Deny the request\} \label{25}
\IF{\textit{Sol:= true}} \label{17}
\RETURN $\{y_j, f^{ij}_{uv}\}$ \{Accept the placement\} \label{18}
\ELSE \label{19}
\STATE $\{\forall{y_j} :=0, \forall{f^{ij}_{uv}} :=0\}$ \label{20}
\RETURN $\{y_j, f^{ij}_{uv}\}$ \{Reject the placement\} \label{21}
\ENDIF \label{22}


\end{algorithmic}
\end{algorithm}

% Since after solving the LP model, the fractional resulting variables do not determine a valid placement for the gateways, we use a deterministic LP-based rounding algorithm to derive integer values for variables.

% \subsection{Load Balancing}
% To balance the flow on the gateways we inject a new constraint to the model. We will force the load difference between any two potential gateways to be less than a certain amount. We refer to this amount by $load_thr$ which is set prior to design of the model. The constraint that carries our load balancing requirement is represented in the following set of constraint: 

% \begin{equation}
%   y_jy_k |\sum_{i\in I}{a_ix_{ij}}-\sum_{i\in I}{a_ix_{ik}}| \leq thr\; \quad \forall j,k\in J
% \end{equation}
% To linearize the above constraint, we introduce a large enough constant $M$ and rewrite the above set of constraints as the two following ones.


% \begin{equation}
%     \sum_{i\in I}{a_ix_{ij}}-\sum_{i\in I}{a_ix_{ik}} \leq (2- y_j-y_k)M + thr\; \quad \forall j,k\in J
% \end{equation}

% \begin{equation}
%         \sum_{i\in I}{a_ix_{ik}}-\sum_{i\in I}{a_ix_{ij}} \leq (2- y_j-y_k)M + thr\; \quad \forall j,k\in J
% \end{equation}
% The constraints imply that for any two pair of gateways the load difference is less than the maximum value allowed, otherwise the constraints are void. 

\subsection{JSGPR-LM MILP Formulation}

We define a new term $l_{max}$ to represent the maximum of assigned traffic to a gateway, among all the gateways in the optimal placement. In order to minimize the forwarding latency we wish to minimize the value of $l_{max}$. Hence, we will add $l_{max}$ as an additional term to the objective function. The new objective function will look like: 

\begin{equation}
    % \textbf{Minimize} \quad(1-\phi)\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
    % \label{obj}
        \textbf{Minimize} \quad(\sum_{j \in J}c_jy_{j}+\phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}) + \alpha l_{max}\;
    \label{objlm}
\end{equation}

Where $\alpha$ is a constant factor determining the balance between the two terms of the objective function. To ensure that the traffic assigned to each gateway does not exceed $l_{max}$, we add the following set of constraints to our model:

\begin{equation}
         \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq l_{max}\; \quad \forall j \in J 
\end{equation}

The resulted optimization problem aims to minimize the load of the gateways in conjunction with the cost of the gateway deployment. 

==> formulation_old2.tex <==
\section{Problem Formulation}
\label{sec:problem}
\subsection{Satellite GW placement problem MILP Formulation I as CFLP}
In order to formulate the  problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{x}$, where $x_{ij}$ expresses the fraction of traffic demand originating at $i$ passing through gateway $j$.
\end{itemize}

 \vspace{2mm}
 \noindent\textbf{Objective function:}
 \begin{equation}
     \textbf{Minimize} \quad \sum_{j\in J}c_j {y_j} + \sum_{i \in I}\sum_{j \in J}{c_{ij} a_{i}x_{ij}}
 \end{equation}

 \begin{equation}
     \sum_{i \in V}{x_{ij}} = 1,\; \quad \forall j \in V
     \label{c1}
 \end{equation}

 \begin{equation}
     x_{ij}\leq y_j, \; \quad \forall i,j \in V
     \label{c2}
 \end{equation}
 
  \begin{equation}
     \sum_{i \in V}a_i {x_{ij}} \leq q_j y_j,\; \quad \forall j \in V
     \label{c3}
 \end{equation}

\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1a}
\end{equation}

\begin{equation}
    \quad 1 \geq x_{ij} \geq 0,\; \quad \forall i \in I, j \in J
    \label{dom2a}
\end{equation}


The objective function minimizes the total cost; which comprises of two terms: the first one represents the cost of installing and opening a gw where $c_j$ denotes the cost of installing and opening a gw at location $j$, the second term accounts for the demand allocation cost, 
where $c_{ij}$ denotes the cost of supplying by gw j the fraction $x_{ij}$  of the demand $a_i$ originating at $i$. Constraint set \ref{c1} assures that traffic demands are supported through the gws, while constraint set \ref{s2} assures that demands are only served by open gws. Constraints \ref{c3} state the capacity constraints for the facilities. The domains of yi and xij variables are defined in constraints \ref{dom1} and \ref{dom2}, respectively. The UFLP is modeled by dropping constraints \ref{c3}.

\subsection{Satellite GW placement problem and routing MILP Formulation I as CFLP}
In order to formulate the  problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{x}$, where $x_{ij}$ expresses the fraction of traffic demand originating at $i$ passing through gateway $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the amount of traffic demand originating at $i$ assigned to gateway $j$ passing through the link $(u,v)$.
\end{itemize}
 \vspace{2mm}
 \noindent\textbf{Objective function:}
 \begin{align}
     \textbf{Minimize} \quad \sum_{j\in J}c_j {y_j} + \sum_{i \in I}\sum_{j \in J}{c_{ij} a_{i}x_{ij}} + \sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}
 \end{align}
 \noindent\textbf{Demand Constraints:}
 \begin{align}
     \sum_{i \in V}{x_{ij}} = 1,\; \quad \forall j \in V
     \label{c1b}
 \end{align}
 \noindent\textbf{Feasibility Constraints:}
 \begin{align}
     x_{ij}\leq y_j, \; \quad \forall i,j \in V
     \label{c2b}
 \end{align}
\begin{align}
     f_{uv}^{ij} \leq a_i x_{ij}, \; \quad \forall i,j \in V
     \label{c3b}
 \end{align}
  \noindent\textbf{Capacity Constraints:}
  \begin{align}
     \sum_{i \in V}a_i {x_{ij}} \leq q_j y_j,\; \quad \forall j \in V
     \label{c4b}
 \end{align}
 \begin{align}
     \sum_{i \in V} \sum_{j \in V} f_{uv}^{ij}  \leq q_{uv}\; \quad \forall j \in V
     \label{c5b}
 \end{align}
  \noindent\textbf{Flow Constraints: }
 \begin{align}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad a_i x_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1b}
\end{align}
\begin{align}
        &\quad \sum_{v \in V: (v,u) \in L}\sum_{j\in J}f^{ij}_{vu} - \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} = a_i x_{iu}\; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i
    \label{flow2b}
\end{align}
%%%%%%%%%%%%%%%%%%
\noindent\textbf{Domain Constraints: }
\begin{align}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1b}
\end{align}
\begin{align}
    \quad  x_{ij} \in \{0, 1\},\; \quad \forall i \in I, j \in J
    \label{dom2b}
\end{align}
\begin{align}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
    \label{dom3b}
\end{align}

The objective function minimizes the total cost; which comprises of three terms; the first one represents the cost of installing and opening a gw at location $j$. The second term accounts for the demand allocation cost, where $c_{ij}$ denotes the cost of supplying by gw j the fraction $x_{ij}$  of the demand $a_i$ originating at $i$. The last term corresponds to the transport/connection cost from the demand originating at $i$ to its assigned gw $j$, 

Constraints set \ref{c1b} assures that traffic demands are supported by the selected gateways. Feasibility constraints set \ref{c2b} make sure that demands are only served by open gateways, while in \ref{c3b} the amount of traffic from the demand originating at $i$ assigned to gateway $j$ passing through the link $(u,v)$ cannot exceed the requested traffic demand $a_i$.  Constraints \ref{c4b} and \ref{c5b} state the capacity constraints for the gateways and the links. Constraints \ref{flow1b} and ref{flow2b} enforce the flow conservation.
The domains of $y_i$, $x_{ij}$ and $f_{uv}^{ij}$ variables are defined in constraints \ref{dom1}, \ref{dom2}, \ref{dom3}, respectively. 

In the aforementioned formulation we can alleviate the constraints set \ref{c4b} if we do not consider any other (e.g., maximum CPU load) on the potential gateways, as well as the $2^{nd}$ term of the objective function if there is no demand allocation cost.





//////////////////////////////////////////////////////
\subsection{JSGPR MILP Formulation II}
In order to formulate the JSGPR problem as a MILP we consider 
\begin{itemize}
    \item The set of binary variables $\textbf{y}$, where $y_j$ expresses the placement of a gateway at node $j$.
    \item The set of continuous variables $\textbf{f}$, where $f_{uv}^{ij}$ expresses the traffic rate passing through the link $(u,v)$ corresponding to flow $i\rightarrow j$.
\end{itemize}

The MILP formulation is as follows:
%as a mixed integer-linear program (MILP) which will follow. 

% \vspace{2mm}
% \noindent\textbf{Objective function:}
% \begin{equation}
%     \textbf{Minimize} \quad \sum_{i\in V}{x_i} + 1/N\sum_{n \in V}\sum_{ij \in E}{z_n^{ij}d_{ij}}
% \end{equation}

% \begin{equation}
%     \sum_{i \in V}{y_{ij}} = 1,\; \quad \forall j \in V
% \end{equation}

% \begin{equation}
%     y_{ij}\leq x_i, \; \quad \forall i,j \in V
% \end{equation}

% \begin{equation}
%     \sum_{iv \in E}{z^{iv}_{j}} - \sum_{ui \in E}{z^{ui}_{j}}  = y_{ij}. \; \quad \forall i,j \in V
% \end{equation}

% \vspace{2mm}
% \noindent\textbf{Objective: }
% \begin{equation}
%     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
% \end{equation}


% \noindent\textbf{Demand Guarantee Constraints: }
% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
% \end{equation}

% \noindent\textbf{Feasibility Guarantee Constraints: }
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}a_ix_{ij} \leq b_jy_j,\; \quad \forall j \in J 
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq a_ix_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% \end{equation}

% \noindent\textbf{Link Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
% \end{equation}

% \noindent\textbf{Flow Constraints: }
% \begin{equation}
%     \quad a_ix_{ii} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + a_ix_{iu}, \; \\ 
%         & \quad \forall i \in I, u \in V,  u \neq i
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

% \begin{equation}
%     \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
% \end{equation}

% \begin{equation}
%     \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
% \end{equation}


% \newpage

\vspace{2mm}
\noindent\textbf{Objective: }
\begin{equation}
    \textbf{Minimize} \quad%(1-\phi)%
    \sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv} \;
    \label{obj}
    %     \textbf{Minimize} \quad\sum_{j \in J}c_jy_{j}\;
    % \label{obj}
\end{equation}


\noindent\textbf{Demand Guarantee Constraints: }
\begin{equation}
    \quad\sum_{j \in J}\sum_{u \in V} f^{ij}_{uj} = a_i,\; \quad \forall i \in I 
    \label{demgar}
\end{equation}

\noindent\textbf{Feasibility Guarantee Constraints: }
\begin{equation}
    \quad \sum_{u \in V} f^{ij}_{uj} \leq y_j a_i,\; \quad \forall i \in I, \forall j \in J 
    \label{leq}
\end{equation}

\noindent\textbf{Delay Guarantee Constraints:}
\begin{equation}
    \quad \sum_{j \in J}\sum_{uv \in L}\frac{f^{ij}_{uv}}{a_i}d_{uv}\leq d_{max} \; \quad \forall{i \in I}
    \label{delgar}
\end{equation}

% \noindent\textbf{Node Capacity Constraints: }
% \begin{equation}
%     \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq b_jy_j,\; \quad \forall j \in J 
%     \label{cap}
% \end{equation}

% \noindent\textbf{Link-Node Capacity Constraints: }
% \begin{equation}
%     \quad f^{ij}_{uv} \leq \sum_{u \in V} f^{ij}_{uj},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
%     \label{maxflow}
% \end{equation}

\noindent\textbf{Link Capacity Constraints: }
\begin{equation}
    \quad \sum_{i \in I}\sum_{j \in J}f^{ij}_{uv} \leq q_{uv},\; \quad \forall uv \in L
    \label{linkcap}
\end{equation}

\noindent\textbf{Flow Constraints: }
\begin{equation}
    % \quad \sum_{u \in V} f^{ii}_{ui} + \sum_{v\in V: iv \in L}\sum_{j \in J}f^{ij}_{iv} = a_i,\; \quad \forall i \in I, i \neq j
        \quad f^{ii}_{ii} + \sum_{v\in V: iv \in L}\sum_{j\neq i \in J }f^{ij}_{iv} = a_i,\; \quad \forall i \in I
    \label{flow1}
\end{equation}

\begin{equation}
    \begin{aligned}
        % &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} + \sum_{u \in V} f^{iu}_{uu}, \; \\ 
        % & \quad \forall i \in I, u \in V,  u \neq i
        &\quad \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{vu} = \sum_{v \in V: (u,v) \in L}\sum_{j\in J}f^{ij}_{uv} \; \\ 
& \quad \forall i \in I, j \in J, u \in V,  u \neq i
    \end{aligned}
    \label{flow2}
\end{equation}

% \begin{equation}
%     \quad x_{ij} \in [0, 1],\; \quad \forall i \in I, j \in J
% \end{equation}

\begin{equation}
    \quad y_{j} \in \{0, 1\},\; \quad \forall j \in J
    \label{dom1}
\end{equation}

\begin{equation}
    \quad f_{uv}^{ij} \geq 0,\; \quad \forall uv \in L, i \in I, j \in J
    \label{dom2}
\end{equation}

\vspace{2mm}
% The first term of the objective function \eqref{obj} is the cost associated with the deployment of the gateways while the second term is the average end-to-end delay of all the flows which traverse the network.  We aim at minimizing the objective function seeking a trade-off between the two terms. The trade-off factor in the objective function is denoted by $\phi$.
The objective function \eqref{obj} is the total cost of the process, consisting of the gateway deployment cost and the bandwidth cost
Constraints \eqref{demgar} are to ensure that the traffic demand for each node is satisfied using one or multiple gateways. Constraints \eqref{leq} allow for the formation of the flow $i\rightarrow j$ only if a gateway is placed at node $j$, while constraints \eqref{delgar} will guarantee that the average end-to-end delay for each demand point will not exceed a pre-defined upper bound $d_{max}$.
% , while constraints \eqref{cap} ensure that the load on each gateway is less than the capacity of the gateway (i.e. less than the capacity of the gateway-satellite node.)
% By constraints \eqref{maxflow}, the rate that each link $(u,v)$ allocates to flow $i\rightarrow j$ is at most equal to the part of the demand of node $i$ which gateway $j$ is responsible for. 
Constraints \eqref{linkcap} make sure that the resources allocated by each link does not exceed the capacity of that link. Constraints \eqref{flow1} and \eqref{flow2}  enforce the flow conservation; i.e. the inbound traffic to a switch must be equal to its outbound traffic. Finally, the  constraints \eqref{dom1}, and \eqref{dom2} express the domain requirements for the variables $\textbf{y}$, and $\textbf{f}$ respectively.

% We also define another notation which does not show up in the problem setup but becomes useful for further discussions. Let $\textbf{x}$ be a set of $x_{ij}$ variables which represent the portion of the traffic originated by node $i$ which is going to be gatewayed to the satellite through gateway $j$. More precisely we write: 
% \begin{equation}
%     x_{ij} = \frac{\sum_{u \in V}{f^{ij}_{uj}}}{a_i}
%     \label{aux}
% \end{equation}
% Where $0\leq x_{ij}\leq1$. Utilizing \eqref{aux}, a few of the constraints in the above-mentioned minimization problem, including \eqref{demgar}, and \eqref{leq}, could be written in the somewhat more intuitive following form:

% % and \eqref{maxflow}, 

% \begin{equation}
%     \quad\sum_{j \in J}x_{ij} = 1,\; \quad \forall i \in I 
%     \label{aux1}
% \end{equation}
% \begin{equation}
%     \quad x_{ij} \leq y_j,\; \quad \forall i \in I, \forall j \in J
%     \label{aux2}
% \end{equation}
% % \begin{equation}
% %     \quad f^{ij}_{uv} \leq a_i x_{ij},\; \quad \forall uv \in L, \forall i \in I, \forall j \in J 
% %     \label{aux3}
% % \end{equation}

% With this alternative notation, the formulated problem very much looks like a variant of the facility location problem formulated in \cite{Bell}; Utilizing the flow variables in the described fashion allows for path splitting which improves the flexibility of the network, and the efficiency of link usage.

Since the MILP is known to be NP-hard, the proposed formulation is intractable for larger scale networks. Next we derive an LP model to strike a balance between the time-complexity of the optimization problem and the accuracy of the results.   


% %TABLE///////////////////%

% \begin{table}[h]
% \centering
% \label{table}
% \begin{center}
% {
% \begin{tabularx}{\textwidth}{|c|X|}

% \hline
% Variables & Description\\
% \hline
% %$q_l[i]$ & Location of the UAV l at timeslot i\\
% $y_j$ & Binary variable determining whether or not a gateway is placed at node $j$. \\
% % $ $ & kjh\\
% $x_{ij}$ & Continuous variable in [0, 1] determining the portion of demanded traffic for node i, which is routed through node j. \\
% $f_{uv}^{ij}$ & The flow passing through the link $(u,v)$ corresponding to node $i$ destined at gateway j.\\
% \hline
% Parameters & Description\\
% \hline
% $a_i$ & Overall traffic generated at node $i$ \\
% $c_j$ & The cost of placing a gateway at node $j$\\
% $d_{uv}$ & The delay corresponding to routing packets through the link $(u,v)$\\
% $q_{uv}$, &Flow capacity of the link $(u,v)$ \\
% %$\rho_0$ & Channel power gain at the reference distance of 1m\\
% %$\gamma_{min}$ & Minimum received SNR for a successful transmission\\
% %$\sigma_n^2$ & Thermal noise power\\
% %$E$ & Transmission power of the nodes\\
% %$d_{min}$ & minimum allowed distance between two UAVs\\
% \hline
% \end{tabularx}}
% \end{center}
% \caption{Variables and Parameters Description}
% \end{table}


\subsection{JSGPR-LM MILP Formulation}

We define a new term $l_{max}$ to represent the maximum of assigned traffic to a gateway, among all the gateways in the optimal placement. In order to minimize the forwarding latency we wish to minimize the value of $l_{max}$. Hence, we will add $l_{max}$ as an additional term to the objective function. The new objective function will look like: 

\begin{equation}
    % \textbf{Minimize} \quad(1-\phi)\sum_{j \in J}c_jy_{j} + \phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}d_{uv}f^{ij}_{uv} \;
    % \label{obj}
        \textbf{Minimize} \quad(\sum_{j \in J}c_jy_{j}+\phi\sum_{i \in I}\sum_{j \in J}\sum_{uv \in L}c_{uv}f^{ij}_{uv}) + \alpha l_{max}\;
    \label{objlm}
\end{equation}

Where $\alpha$ is a constant factor determining the balance between the two terms of the objective function. To ensure that the traffic assigned to each gateway does not exceed $l_{max}$, we add the following set of constraints to our model:

\begin{equation}
         \quad \sum_{i \in I}\sum_{u \in V} f^{ij}_{uj} \leq l_{max}\; \quad \forall j \in J 
\end{equation}

The resulted optimization problem aims to minimize the load of the gateways in conjunction with the cost of the gateway deployment. 
